Reinforcing RCTs with Multiple Priors while Learning about External Validity

This paper introduces a framework for incorporating prior information into the design of sequential experiments. These sources may include past experiments, expert opinions, or the experimenter's intuition. We model the problem using a multi-prior Bayesian approach, mapping each source to a Bayesian model and aggregating them based on posterior probabilities. Policies are evaluated on three criteria: learning the parameters of payoff distributions, the probability of choosing the wrong treatment, and average rewards. Our framework demonstrates several desirable properties, including robustness to sources lacking external validity, while maintaining strong finite sample performance.

==> app_GeneralAlphaAsymptotics.tex <==
\section{Proof of Proposition \ref{pro:alpha.asymptotics.general}}
\label{app:General.Bound.alpha}



To show Proposition \ref{pro:alpha.asymptotics.general} we use the following lemmas whose proofs are relegated to Supplemental Material \ref{app:SM_GeneralBoundsAlpha}. The first lemma studies the process $g(Y_{s},D_{s},\theta) : = (1\{D_{s}(x) = d \} ( \ell (Y_{s},\theta)  - E[  \ell (Y_{s},\theta) \mid D_{s}(x)  ]  ) $ for all $s \geq 1$, where the expectation is taken with respect to $P(.|d,x)$ and $\ell(.,\theta) : = \log p_{\theta}(.)/p(. \mid d,x )$ and $p(\cdot | d,x)$ is the true PDF of $Y(d,x)$. 

In what follows, let $B(\theta,\delta)$ as the ball with radius $\delta>0$, centered at $\theta \in \Theta$. 

\begin{lemma}\label{lem:uniform.LLN} 
%	Suppose $\Theta \subseteq \mathbb{R}^{|\Theta|}$ is compact and there exists a $C < \infty$ and $\kappa > 0$ such that $$ \max_{\theta' \in \Theta} E[ \sup_{\theta \in B(\theta',\delta)  }  | \ell(Y(d,x),\theta) - \ell(Y(d,x),\theta') |^{2}  ] \leq C^{2} \delta^{2\kappa},~\forall \delta >0. $$
	Suppose $\Theta \subseteq \mathbb{R}^{|\Theta|}$ is compact and there exists a $\varphi : \mathbb{R}_{+} \rightarrow \mathbb{R}_{+}$ increasing, such that $\varphi(0)=0$  and $$ \max_{\theta' \in \Theta} E[ \sup_{\theta \in B(\theta',\delta)  }  | \ell(Y(d,x),\theta) - \ell(Y(d,x),\theta') |^{2}  ] \leq \varphi(\delta)^{2},~\forall \delta >0. $$
	 Then there exists a $C >0$ such that for any $t \in \mathbb{N}$ and $\gamma > 0$,  	
	\begin{align*}
		\mathbf{P} \left( \sup_{\theta \in \Theta } |  t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta)  | \geq \sqrt{1/(2C \gamma) } \sqrt{ \Lambda(t, |\Theta|)  }  \right) \leq \gamma
	\end{align*} 
where $\Lambda(t,|\Theta|) : =  \min_{\delta \geq 0} ( t^{-1} \delta^{-|\Theta|} + \varphi(\delta)) $ and is decreasing in $t$ and increasing in $|\Theta|$ and $\lim_{t\rightarrow \infty} \Lambda(t,|\Theta|) = 0$.
\end{lemma}

The following lemma provides a non-asymptotic bound for the ratio of the weights for any two models. In particular, it relates the weights, $\alpha^{o}_{t}$, with the Laplace transform of the CDF $$ u \mapsto G^{o}_{d,x}(u) : = \mu_{0}^{o}(d,x) (  KL_{d,x}(\theta) \leq u   ). $$ To ou knowledge, this result is new and might be of independent interest.

\begin{lemma}\label{lem:alpha.asymptotics.general}
		Take any $o,o' \in \{0,...,L\}$ and $(d,x) \in \mathbb{D}\times \mathbb{X}$. Suppose $\Theta \subseteq \mathbb{R}^{|\Theta|}$ is compact and there exists a $\varphi : \mathbb{R}_{+} \rightarrow \mathbb{R}_{+}$ increasing, such that $\varphi(0)=0$ and $$ \max_{\theta' \in \Theta} E[ \sup_{\theta \in B(\theta',\delta)  }  | \ell(Y(d,x),\theta) - \ell(Y(d,x),\theta') |^{2}  ] \leq \varphi(\delta)^{2},~\forall \delta >0. $$
		Then, for any $\gamma > 0$,
		\begin{align*}
			\frac{\alpha^{o}_{t}(d,x)}{\alpha^{o'}_{t}(d,x)} \leq \frac{ \int G^{o}_{d,x}(u)  e^{-N_{t}(d,x) u} du  }{ \int G^{o'}_{d,x}(u)  e^{-N_{t}(d,x) u} du } e^{t r_{t}}~\forall t,
		\end{align*}
		with probability larger than $1-\gamma$,  where $r_{t} : =  \sqrt{ 1/(2C\gamma) } \sqrt{ \Lambda(t,|\Theta|)  }  $ and $C$ is as in lemma \ref{lem:uniform.LLN}.
\end{lemma}




\begin{proof} [Proof of Proposition \ref{pro:alpha.asymptotics.general}] 
	
	Suppose the conditions in Lemma \ref{lem:alpha.asymptotics.general} hold (we show they do towards the end of the proof). 
	
	Throughout, fix a $(d,x) \in \mathbb{D}\times \mathbb{X}$ and $o,o' \in \{0,...,L\}$. 
	
	For any $\gamma>0$, let $O_{t}(\gamma)$ be the set of histories such that 
	\begin{align*}
		\frac{\alpha^{o}_{t}(d,x)}{\alpha^{o'}_{t}(d,x)} \leq \frac{ \int G^{o}_{d,x}(u)  e^{-N_{t}(d,x) u} du  }{ \int G^{o'}_{d,x}(u)  e^{-N_{t}(d,x) u} du } e^{t r_{t}},
	\end{align*}
	where $(r_{t})_{t}$ is the sequence defined in Lemma \ref{lem:alpha.asymptotics.general}; observe that $r_{t}$ depends on $\gamma$, and thus, so does the set $O_{t}(\gamma)$. By Lemma \ref{lem:alpha.asymptotics.general}, $\mathbf{P}(O_{t}(\gamma)^{C}) \leq  \gamma$ for any $t \in \mathbb{N}$. 
	
	For any $\varepsilon>0$, let $S_{t}(\varepsilon)$ be the set of histories such that $N_{t}(d,x)/t  \geq \iota_{t}(d,x) - \varepsilon$. By Lemma \ref{lem:Azzuma} in Appendix \ref{app:ConcentrationInequalities}, there exists a $t_{\varepsilon}$ such that $\mathbf{P} (S_{t}(\varepsilon) ^{C} ) \leq \varepsilon$ for all $t \geq t_{\varepsilon}$. 
	
	In this case, it follows that for any $\varepsilon>0$ any $\gamma>0$,
	\begin{align*}
		\mathbf{P} \left( 	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq \varepsilon   \right) \leq & \mathbf{P} \left( 	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq \varepsilon  \cap S_{t}(\varepsilon ) \cap O_{t}(\gamma) \right) + \mathbf{P} \left( O_{t}(\gamma )^{C}  \right) + \mathbf{P} \left( S_{t}(\varepsilon )^{C}  \right)
	\end{align*}
	for all $t \in \mathbb{N}$. 
	
	In what follows, take an arbitrary sequence in $O_{t}(\gamma )$. Let $u_{o}(d,x)$ as in the definition. If $u_{o}(d,x) - u_{o'}(d,x) = : A > 0$, then,
	\begin{align*}
		\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq & e^{2 t r_{t} }	\frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right) e^{-N_{t}(d,x)v} dv   } \\
		\leq & e^{2 t r_{t} }	\frac{ N_{t}(d,x) \int_{u_{o}(d,x)}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{u_{o'}(d,x)}^{ u_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)   \leq v \right) e^{-N_{t}(d,x)v} dv   }	\\
		\leq & e^{2 t r_{t} }	\frac{ e^{-N_{t}(d,x) u_{o}(d,x) }   \int_{u_{o}(d,x)}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x} (\theta)   \leq v \right) dv  } { e^{-N_{t}(d,x)  (  m_{o'}(d,x)  + 0.5 A )  } \int_{m_{o'}(d,x)}^{ u_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right)  dv   } \\
		= & e^{ - N_{t}(d,x)  0.5 A + 2 t r_{t}   }   \frac{  \int_{u_{o}(d,x)}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x} (\theta)   \leq v \right) dv  } {  \int_{u_{o'}(d,x)}^{ u_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right)  dv   }
	\end{align*}
	where the last line follows from definition of $A$. 
	
		The fraction in the previous display is a fixed number. Under the set $S_{t}(\varepsilon)$, $\frac{N_{t}(d,x)}{t}  0.5 A + 2 r_{t} \geq (\iota_{t}(d,x) - \varepsilon ) 0.5 A - 2 \varepsilon $. Under the assumption that $\inf_{t} \iota_{t}(d,x) > 0$, there exists a $\bar{\varepsilon}>0$ (not dependant on $t$) such that for any $\varepsilon \leq \bar{\varepsilon}$, $\frac{N_{t}(d,x)}{t}  0.5 A + 2 r_{t} \geq c > 0$. Thus, we obtain $\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } = O( e^{-t c } )$, which in turn implies that 
		for any $\varepsilon \in (0,\bar{\varepsilon})$ any $\gamma>0$,
		\begin{align*}
			\mathbf{P} \left( 	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq \varepsilon   \right) \leq & \mathbf{P} \left( e^{-tc} \geq \varepsilon \right) + \mathbf{P} \left( O_{t}(\gamma )^{C}  \right) + \mathbf{P} \left( S_{t}(\varepsilon )^{C}  \right)
		\end{align*}
		for all $t \in \mathbb{N}$. By choosing $\gamma = \varepsilon$, for any $t \geq \max\{ t_{\varepsilon} , c^{-1}\log 1/\varepsilon  \} $ the RHS is less than $2 \varepsilon $ and the desired result holds. 
		

	
%	
%	
%	XXXXXXXXXXXXXXXXXXXXXXXXXXXX
%	
%	
%	In this case, it follows  that for any $\varepsilon>0$,
%	\begin{align*}
%		\mathbf{P} \left( 	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq \varepsilon   \right) \leq \mathbf{P} \left( 	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq \varepsilon  \cap S_{t}(\varepsilon ) \right) + \mathbf{P} \left( S_{t}(\varepsilon )^{C}  \right)
%	\end{align*}
%	where $S_{t}(\varepsilon )$ is the set such that $N_{t}(d,x)/t  \geq \iota_{t}(d,x) - \varepsilon$ and $r^{-1}_{t} \sup_{\theta \in \Theta}  \left| t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta)   \right| \leq \varepsilon $. By Lemma \ref{lem:uniform.LLN}, Lemma \ref{lem:Azzuma}, $\lim_{t\rightarrow \infty} \mathbf{P} (S_{t}(\varepsilon) ^{C} ) =0$. 
%	
%	In what follows, take an arbitrary sequence in $S_{t}(\varepsilon )$. Let $u_{o}(d,x)$ as in the definition. If $u_{o}(d,x) - u_{o'}(d,x) = : A > 0$, then by Lemma \ref{lem:alpha.asymptotics.general}, 
%	\begin{align*}
%		\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq & e^{2 t r_{t} }	\frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right) e^{-N_{t}(d,x)v} dv   } \\
%		\leq & e^{2 t r_{t} }	\frac{ N_{t}(d,x) \int_{u_{o}(d,x)}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{u_{o'}(d,x)}^{ u_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)   \leq v \right) e^{-N_{t}(d,x)v} dv   }	\\
%		\leq & e^{2 t r_{t} }	\frac{ e^{-N_{t}(d,x) u_{o}(d,x) }   \int_{u_{o}(d,x)}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x} (\theta)   \leq v \right) dv  } { e^{-N_{t}(d,x)  (  m_{o'}(d,x)  + 0.5 A )  } \int_{m_{o'}(d,x)}^{ u_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right)  dv   } \\
%		= & e^{ - N_{t}(d,x)  0.5 A + 2 t r_{t}   }   \frac{  \int_{u_{o}(d,x)}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x} (\theta)   \leq v \right) dv  } {  \int_{u_{o'}(d,x)}^{ u_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right)  dv   }
%	\end{align*}
%	where the last line follows from definition of $A$. 
%	
%	The fraction in the previous display is a fixed number. Under the set $S_{t}(\varepsilon)$, $\frac{N_{t}(d,x)}{t}  0.5 A + 2 r_{t} \geq (\iota_{t}(d,x) - \varepsilon ) 0.5 A - 2 \varepsilon $. Under the assumption that $\inf_{t} \iota_{t}(d,x) > 0$, there exists a $\bar{\varepsilon}>0$ (not dependant on $t$) such that for any $\varepsilon \leq \bar{\varepsilon}$, $\frac{N_{t}(d,x)}{t}  0.5 A + 2 r_{t} \geq c > 0$. Thus, we obtain $\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } = O( e^{-t c } )$, which in turn implies that 
%	\begin{align*}
%		\mathbf{P} \left( 	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq \varepsilon   \right) \leq \mathbf{P} \left(  e^{-t c }  \geq \varepsilon  \right) + \mathbf{P} \left( S_{t}(\varepsilon )^{C}  \right) = o(1),
%	\end{align*}
%	for any $\varepsilon \leq \bar{\varepsilon}$. Thus the desired result follows. 
	
	\bigskip
	
	We now verify that the conditions in Lemma \ref{lem:alpha.asymptotics.general} (and thus, Lemma \ref{lem:uniform.LLN}) hold. $\Theta$ is compact by assumption, so we ``just" need to verify the continuity condition. 
	
	By Assumption, $\theta \mapsto \log p_{\theta}(\cdot)$ is continuous a.s.-$\mathbf{P}$. This implies that $\theta \mapsto \ell(\cdot,\theta)$ is continuous a.s.-$\mathbf{P}$.  Continuous functions over compact sets are uniformly continuous, thus $f(Y(d,x),\delta) : = \sup_{||\theta-\theta'|| \leq \delta} |\ell(Y(d,x),\theta) - \ell(Y(d,x),\theta')| $ converges to 0 as $\delta$ vanishes a.s.-$\mathbf{P}$. By Assumption, $$E[\sup_{\theta \in \Theta} | \log p_{\theta} (Y(d,x))|^{2}   ] < \infty,$$ and thus by the Dominated convergence theorem, $\lim_{\delta \rightarrow 0} E[f(Y(d,x),\delta) ^{2} ] = 0$ as desired.  
	%
	%
	%If $\frac{t r_{t}}{N_{t}(d,x)} = o(1)$ XXX, then if follows that the RHS converges to to zero as $ e^{-N_{t}(d,x) m_{o}(d,x) } / e^{-N_{t}(d,x)  (  m_{o'}(d,x)  + 0.5 A )  }  = o(1)$ and $\int_{m_{o'}(d,x)}^{ m_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{o'}(d,x)(\theta) + \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right)  dv $ converges to $\int_{m_{o'}(d,x)}^{ m_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{o'}(d,x)(\theta) \leq v \right)  dv >0 $.
	%
	%If $m_{o}(d,x) = m_{o'}(d,x) = A>0$ and $\frac{t r_{t}}{N_{t}(d,x)} = o(1)$, then
	%\begin{align*}
	%	& \frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{o}(d,x)(\theta) - \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{o'}(d,x)(\theta) + \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   }  \\
	%	\leq &  \frac{ N_{t}(d,x) \int_{A}^{\infty} G_{o}(d,x)(v) e^{-N_{t}(d,x)v} dv  + \left( \frac{t r_{t}}{N_{t}(d,x)} \right) ^{\rho} C e^{-N_{t}(d,x)A}  } { N_{t}(d,x) \int_{A}^{\infty}  G_{o'}(d,x) (v)  e^{-N_{t}(d,x)v} dv - \left( \frac{t r_{t}}{N_{t}(d,x)} \right) ^{\rho} C e^{-N_{t}(d,x)A}}.  
	%\end{align*}
	%
	%
	%
	%XXX Gaussian 
	%
	%Suppose $KL_{o}(d,x)(\theta) = 0.5(\theta(d,x) - \theta^{\ast}(d,x))^{2}$ and $\mu^{o}_{0}(d,x)$ is Gaussian with mean $\zeta_{0}^{o}(d,x)$ and $1/\nu_{0}^{o}(d,x)$. Then, for any $v \geq 0$, 
	%\begin{align*}
	%	 \mu^{o}_{0}(d,x) \left( KL_{o'}(d,x)(\theta)  \leq v \right) = & \int_{-\sqrt{2v} + \theta^{\ast}(d,x) }^{\sqrt{2v} + \theta^{\ast}(d,x) } \phi(w; \zeta_{0}^{o}(d,x), 1/\nu_{0}^{o}(d,x))dw \\
	%	 = & 2 \Phi( \sqrt{2v} + \theta^{\ast}(d,x) ; \zeta_{0}^{o}(d,x), 1/\nu_{0}^{o}(d,x) )
	%\end{align*}
	%
	%\begin{align*}
	%	\int_{0}^{\infty}  G_{o'}(d,x) (v)  e^{-N_{t}(d,x)v} dv  = \int_{A}^{\infty} 2 \Phi( \sqrt{2v} + \theta^{\ast}(d,x) ; \zeta_{0}^{o}(d,x), 1/\nu_{0}^{o}(d,x) )  e^{-N_{t}(d,x)v} dv  
	%\end{align*}
	%
	%
	%XXXXXXXXXXXXXXXXXXXXXXXXXX
	%
	%
	%Moreover XXXX. 
	%
	%Therefore, Lemma XXX implies that for any $\varepsilon>0$,
	%\begin{align*}
	%	P \left( \left| t^{-1} \sum_{s=1}^{t} g_{o}(Y_{s},D_{s},\theta)   \right| \geq r(t, \varepsilon ) \right) \leq v(t,\varepsilon)
	%\end{align*}
	%where $r(t,\varepsilon) : = XXX$ and $v(t,\varepsilon) : = XXX$. This result and the fact that $\sum_{s=1}^{t} 1\{D_{s} = d \} E [  \ell_{o} (Y_{s},\theta) \mid D_{s} ] = \sum_{s=1}^{t} 1\{D_{s} = d \} E [  \ell_{o} (Y_{s}(d),\theta)  ] = t f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ] $ imply that
	%	\begin{align*}
		%	P \left( \frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq \frac{\int \exp \left\{ t ( f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]  -  r(t, \varepsilon ) )  \right\}   \mu^{o}_{0}(d,x)(d\theta)} {\int \exp \left\{ t ( f_{t}(d) E [  \ell_{o'} (Y(d),\theta)  ]  + r(t, \varepsilon ) ) \right\} \mu^{o'}_{0}(d,x)(d\theta)   } \right) \geq 1 - v(t,\varepsilon) 
		%\end{align*}
		%and 
		%	\begin{align*}
			%	P \left( \frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq \frac{\int \exp \left\{ t ( f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]  +  r(t, \varepsilon ) )  \right\}   \mu^{o}_{0}(d,x)(d\theta)} {\int \exp \left\{ t ( f_{t}(d)  E [  \ell_{o'} (Y(d),\theta)  ]  - r(t, \varepsilon ) ) \right\} \mu^{o'}_{0}(d,x)(d\theta)   } \right) \geq 1 - v(t,\varepsilon) .
			%\end{align*}
			%
			%
			%Observe that
			% \begin{align*}
				%	\int \exp \{ t  f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]  \}  \mu^{o}_{0}(d,x)(d\theta) = & \int_{1}^{\infty} \mu^{o}_{0}(d,x) \left( \exp \{  t  f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ] \} \geq x     \right) dx \\
				%	= & \int_{1}^{\infty} \mu^{o}_{0}(d,x) \left(   t  f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]  \geq (\log x)/(  t  f_{t}(d)  )      \right) dx \\
				%	= & t f_{t}(d)  \int_{0}^{\infty} \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  f_{t}(d) u  \} du  
				%\end{align*}
				%where the 3rd equality follows from a change of variables $u = (\log x)/(  t  f_{t}(d)  )$ where 
				% $ t f_{t}(d) \exp\{  t  f_{t}(d) u  \} du = dx $. Thus,
				%\begin{align*}
				%	\frac{\int \exp \left\{ t  f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]   \right\}   \mu^{o}_{0}(d,x)(d\theta)} {\int \exp \left\{ t f_{t}(d)  E [  \ell_{o'} (Y(d),\theta)  ]  \right\} \mu^{o'}_{0}(d,x)(d\theta)   } = \frac{ \int_{0}^{\infty} \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  f_{t}(d) u  \}    du   } {  \int_{0}^{\infty} \mu^{o'}_{0}(d,x) \left(   E [  \ell_{o'} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  f_{t}(d) u  \}  du   }  .
				%\end{align*}
				%
				%Hence, since $KL_{o}(d,x)(\theta) : = - E [  \ell_{o} (Y(d),\theta)  ]$ it follows that, with probability greater or equal to $1-v(\varepsilon,t)$,
				%
				%%\begin{align*}
				%%	 \frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq  \frac{ \int_{0}^{\infty} \mu^{o}_{0}(d,x) \left(   KL_{o}(d,x)(\theta)  \leq -u   \right)  \exp\{  t  f_{t}(d) u  \}    du   } {  \int_{0}^{\infty} \mu^{o'}_{0}(d,x) \left(   KL_{o'}(d,x)(\theta) \leq -u   \right)  \exp\{  t  f_{t}(d) u  \}  du   }  \exp\{ 2t r(t, \varepsilon )   \}
				%%\end{align*}
				%\begin{align*}
				%	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq  \frac{ \int_{0}^{\infty} \mu^{o}_{0}(d,x) \left(   KL_{o}(d,x)(\theta)  \leq u   \right)  \exp\{  -t  f_{t}(d) u  \}    du   } {  \int_{0}^{\infty} \mu^{o'}_{0}(d,x) \left(   KL_{o'}(d,x)(\theta) \leq u   \right)  \exp\{  -t  f_{t}(d) u  \}  du   }  \exp\{ 2t r(t, \varepsilon )   \}
				%\end{align*}
				%and
				%\begin{align*}
				%	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq  \frac{ \int_{0}^{\infty} \mu^{o}_{0}(d,x) \left(  KL_{o}(d,x)(\theta)  \leq u   \right)  \exp\{  - t  f_{t}(d) u  \}    du   } {  \int_{0}^{\infty} \mu^{o'}_{0}(d,x) \left(   KL_{o'}(d,x)(\theta) \leq u   \right)  \exp\{  - t  f_{t}(d) u  \}  du   }  \exp\{ -2t r(t, \varepsilon )   \}.
				%\end{align*}
				%
				%$u \mapsto \mu^{o}_{0}(d,x) \left(   KL_{o}(d,x)(\theta)  \leq u   \right)  = : G_{o}(d,x)(u)$ is a CDF. 
				
				%
				%XXXXXXXXXXXXXXXXXXXXXXXXXXXXX
				%
				%
				%XXXXX
				%
				%If support are different: 
				%
				%\begin{align*}
				%	\frac{\int \exp \left\{ t  f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]   \right\}   \mu^{o}_{0}(d,x)(d\theta)} {\int \exp \left\{ t f_{t}(d)  E [  \ell_{o'} (Y_{s}(d),\theta)  ]  \right\} \mu^{o'}_{0}(d,x)(d\theta)   } \leq & \frac{ \int_{0}^{A} \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  f_{t}(d) u  \}    du   } {  \int_{A+\delta}^{B} \mu^{o'}_{0}(d,x) \left(   E [  \ell_{o'} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  f_{t}(d) u  \}  du   }  \\
				%	\leq &  \frac{  \exp\{  t  f_{t}(d) A  \}   \int_{0}^{A} \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq u   \right)   du   } {  \exp\{  t  f_{t}(d) (A + \delta)  \}    \int_{A+\delta}^{B} \mu^{o'}_{0}(d,x) \left(   E [  \ell_{o'} (Y(d),\theta)  ]  \geq u   \right)  du   } 
				%\end{align*}
				%
				%If support are the same:
				%
				%\begin{align*}
				%& \frac{ \int_{0}^{A} \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  ( f_{t}(d) u  + r(t,\epsilon) )  \}    du   } {  \int_{0}^{A} \mu^{o'}_{0}(d,x) \left(   E [  \ell_{o'} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t ( f_{t}(d) u  - r(t,\epsilon) )   \}  du   }  \\
				%= & \frac{ \int_{0}^{  t(  r(t,\epsilon)  + A f_{t}(d))  } \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq (v/t  - r(t,\epsilon) )/ f_{t}(d)   \right)  \exp\{  v   \}    dv  } {  \int_{0}^{ t ( - r(t,\epsilon)  + A f_{t}(d) ) } \mu^{o'}_{0}(d,x) \left(   E [  \ell_{o'} (Y(d),\theta)  ]  \geq (v/t  + r(t,\epsilon) )/ f_{t}(d)   \right)  \exp\{  v   \}  dv   } 
				%\end{align*}
				%
				%
				%XXXXXXXXXXXXX
				%
				%Moreover, 
				%\begin{align*}
				%	\int \exp \left\{ t ( f_{t}(d) E [  \ell_{o} (Y_{s}(d),\theta)  ]  +  r(t, \epsilon ) )  \right\}   \mu^{o}_{0}(d,x)(d\theta) \leq \exp \left\{ t ( f_{t}(d) \max_{\theta \in \Theta_{o}}   E [  \ell_{o} (Y_{s}(d),\theta)  ]  +  r(t, \epsilon ) )  \right\}
				%\end{align*}
				%and
				%\begin{align*}
				%	\int \exp \left\{ t ( f_{t}(d) E [  \ell_{o} (Y_{s}(d),\theta)  ]  +  r(t, \epsilon ) )  \right\}   \mu^{o}_{0}(d,x)(d\theta) \geq \exp \left\{ t ( f_{t}(d) \min_{\theta \in \Theta_{o}(\delta)  }   E [  \ell_{o} (Y_{s}(d),\theta)  ]  +  r(t, \epsilon ) )  \right\} \mu_{0}^{o}( \Theta_{o}(\delta)  )
				%\end{align*}
				% where, for any $\delta> 0$, $\Theta_{o}(\delta)  : = \{ \theta \in \Theta_{o} \colon E [  \ell_{o} (Y_{s}(d),\theta)  ]  \geq  \max_{\theta \in \Theta_{o}}   E [  \ell_{o} (Y_{s}(d),\theta)  ]  - \delta     \}$.
				% 
				% XXXXXXX
				% 
			\end{proof}
			




%\subsection{Proof of Supplemental Lemmas}
%
%\begin{proof}[Proof of Lemma \ref{lem:uniform.LLN} ]	
%	Henceforth, we omit the notation "$x$" from the quantities as there is no risk of confusion. Let $\mathcal{F}^{s}$ denote the $\sigma$-algebra generated by $(D_{1},...,D_{s},Y_{1},...,Y_{s-1})$. We now show that for each $\theta \in \Theta$, $(g(Y_{s},D_{s},\theta))_{s}$ is a MDS with respect to aforementioned $\sigma$-algebra. To do this, note that 
%	\begin{align*}
%		E[ g(Y_{s},D_{s},\theta) \mid  \mathcal{F}^{s} ] = 1\{D_{s} = d \}  E[ \ell (Y_{s},\theta)  - E[  \ell (Y_{s},\theta) \mid D_{s} ] \mid  \mathcal{F}^{s} ].
%	\end{align*}
%	Observe that $E[ \ell (Y_{s},\theta)  \mid  \mathcal{F}^{s} ] = E[ \ell (Y_{s},\theta)  \mid  D_{s} ] $ because $Y_{s}$ is independent of the whole past once we condition on $D_{s}$. Since $E[[  \ell (Y_{s},\theta) \mid D_{s} ] \mid  \mathcal{F}^{s} ] = E [  \ell (Y_{s},\theta) \mid D_{s} ] $, it follows that $E[ g(Y_{s},D_{s},\theta) \mid  \mathcal{F}^{s} ]  = 0$. 
%	
%	
%	Since $\Theta$ is assumed to be compact, for any $\delta>0$, there exists a $L_{\delta}$ such that $\Theta \subseteq \cup_{l =1}^{L} B(\theta_{l},\delta)$ where $B(\theta,\delta)$ is a $\delta$-radius ball with center $\theta$. Indeed, let $L_{\delta}$ be the smallest number of balls of radius $\delta$ needed to cover the set, and as $\Theta \subseteq \mathbb{R}^{|\Theta|}$, it follows that $L_{\delta} \leq C \delta^{-|\Theta|}$ where $C$ is an universal constant. %; see XXX. 
%	Thus, for any $t$ and any $\delta>0$,
%	\begin{align*}
%		\sup_{\theta \in \Theta}  |t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta) | \leq &	\max_{l \in \{1,...,L_{\delta} \}}  |t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta_{l}) |  \\
%		& +  	\max_{l \in \{1,...,L_{\delta} \}}  	\sup_{\theta \in B(\theta_{l},\delta)  }  |t^{-1} \sum_{s=1}^{t} \{  g(Y_{s},D_{s},\theta) - g(Y_{s},D_{s},\theta_{l})\} | .
%	\end{align*}
%	
%	%	We now show that for any $\varepsilon$, there exists a $\delta$ (not dependening on $t$ nor $l$) such that $$E[ \sup_{\theta \in B(\theta_{l},\delta)  }  |t^{-1} \sum_{s=1}^{t} \{  g_{o}(Y_{s},D_{s},\theta) - g_{o}(Y_{s},D_{s},\theta_{l})\} | ]  \leq  \varepsilon .$$ This follows because, by assumption XXX, 
%	By the triangle inequality and simple algebra, for any $t$, any $\delta>0$ and any $l \in \{1,...,L_{\delta}\}$,
%	\begin{align*}
%		 \sqrt{E[ \sup_{\theta \in B(\theta_{l},\delta)  }  |t^{-1} \sum_{s=1}^{t} \{  g(Y_{s},D_{s},\theta) - g(Y_{s},D_{s},\theta_{l})\} |^{2}  ] } &	\leq  t^{-1} \sum_{s=1}^{t} \sqrt{E[ \sup_{\theta \in B(\theta_{l},\delta)  }  | g(Y_{s},D_{s},\theta) - g(Y_{s},D_{s},\theta_{l}) |^{2}  ] }\\
%	%	& \leq  2 t^{-1} \sum_{s=1}^{t } \sqrt{E[ \sup_{\theta \in B(\theta_{l},\delta)  }  | \ell(Y_{s}(d,x),\theta) - \ell(Y_{s}(d,x),\theta_{l})) |^{2}  ] } \\
%		& \leq  2 \sqrt{E[ \sup_{\theta \in B(\theta_{l},\delta)  }  | \ell(Y(d,x),\theta) - \ell(Y(d,x),\theta_{l})) |^{2}  ]} 			 
%	\end{align*}
%	where the last line follows from IID-ness of $Y(d,x)$. By Assumption, the RHS is less than $\varphi( \delta ) $. 
%	
%	By the Martingale difference property, for any $t$ and any $\delta>0$, 
%	\begin{align*}
%		E[( 	\max_{l \in \{1,...,L_{\delta} \}}  |t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta_{l}) |  )^{2} ] \leq & L_{\delta} t^{-1} \max_{1 \leq s \leq t} E[(  g(Y_{s},D_{s},\theta_{l})  )^{2} ] \leq C L_{\delta} t^{-1} \max_{1 \leq s \leq t} E[(  \ell(Y(d,x),\theta_{l})  )^{2} ]
%	\end{align*} 
%	for some universal constant $C$. Compactness of $\Theta$ and the continuity assumption imply that $\max_{l} E[(  \ell(Y(d,x),\theta_{l})  )^{2} ] \leq C$ for some finite constant. 
%	
%	Then, by the Markov inequality, for any $\varepsilon>0$, any $t$ and any $\delta>0$,
%	\begin{align*}
%		\mathbf{P} \left( \sup_{\theta \in \Theta } |  t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta)  | \geq \varepsilon   \right) \leq & C ( \varepsilon^{-2} t^{-1} L_{\delta} +  \varepsilon^{-1} \varphi( \delta )  ) \leq C \varepsilon^{-2} (  t^{-1} \delta^{-|\Theta|} +  \varphi( \delta )   ) 
%	\end{align*}
%	
%	For any $t$, choose $\delta$ as the argmin of $\Lambda(t,|\Theta|) : =  \min_{\delta \geq 0} ( t^{-1} \delta^{-|\Theta|} + \varphi(\delta)) $. %This implies that $  t^{-1} \delta^{-|\Theta|} +  \delta^{\kappa} = 2 t^{-\frac{\kappa}{ |\Theta| + \kappa }}$. 
%	Observe that $\Lambda(.,.)$ is decreasing in $t$ and increasing in $|\Theta|$ and $\lim_{t\rightarrow \infty} \Lambda(t,|\Theta|) = 0$; the first property is straightforward and the second one follows because $t^{-1} \delta^{-|\Theta|} + \varphi(\delta)$ converges to $\varphi(\delta)$ (pointwise) and $\varphi(0) = 0$. 
%	
%	
%	Hence, by choosing $\varepsilon = \sqrt{(0.5/C) M} \sqrt{ \Lambda(t,|\Theta|)  } $, the previous display implies that for any $M>0$ 
%	\begin{align*}
%			\mathbf{P} \left( \sup_{\theta \in \Theta } |  t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta)  | \geq \sqrt{(0.5/C) M} \sqrt{ \Lambda(t,|\Theta|)  }    \right) \leq M^{-1} 
%	\end{align*} 
%	for any $t$. Thus, by setting $r_{t} = \sqrt{(0.5/C) M} \sqrt{ \Lambda(t,|\Theta|)  } $ and re-defining $M$ as $1/\gamma$ the desired result follows. 
%\end{proof}
%
%\begin{proof} [Proof of Lemma  \ref{lem:alpha.asymptotics.general}] 
%	For any $(d,x) \in \mathbb{D} \times \mathbb{X}$ and any $o,o' \in \{0,...,L\}$ observe that 
%	\begin{align*}
%		\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } = \frac{\int \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta)  \right\}   \mu^{o}_{0}(d,x)(d\theta)} {\int \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell(Y_{s},\theta)  \right\} \mu^{o'}_{0}(d,x)(d\theta)   }
%	\end{align*}
%	where $\ell(.,\theta) : = \log p_{\theta}(.)/p(. \mid d,x )$ and $p(\cdot | d,x)$ is the true PDF of $Y(d,x)$. Moreover,
%	\begin{align*}
%		\int \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta)   \right\}   \mu^{o}_{0}(d,x)(d\theta) 	= & \int_{1}^{\infty}  \mu^{o}_{0}(d,x) \left(  \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta)  \right\} \geq u \right) du \\
%		= & N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( - \frac{N_{t}(d,x) }{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta) } \leq v \right) e^{-N_{t}(d,x)v} dv
%	\end{align*}
%	where the second equality is obtained by a change of variables $v = - N^{-1}_{t}(d,x) \log u$. 
%	
%	In addition, note that
%	\begin{align*}
%		N^{-1}_{t}(d,x)  \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta) = & \frac{t}{N_{t}(d,x)} t^{-1}  \sum_{s=1}^{t}  g(Y_{s},D_{s},\theta) +	N^{-1}_{t}(d,x)  \sum_{s=1}^{t} 1\{D_{s}(x) = d \} E[  \ell (Y_{s},\theta) \mid D_{s}  ] \\
%		= & \frac{t}{N_{t}(d,x)} t^{-1}  \sum_{s=1}^{t}  g(Y_{s},D_{s},\theta)  + E[  \ell (Y(d,x),\theta)  ] 
%	\end{align*}
%	where $g(Y_{s},D_{s},\theta) : = (1\{D_{s}(x) = d \} ( \ell (Y_{s},\theta)  - E[  \ell (Y_{s},\theta) \mid D_{s}(x)  ]  ) $  and the last line follows because $1\{D_{s}(x) = d \} E[  \ell (Y_{s},\theta) \mid D_{s}(x)  ] = 1\{D_{s}(x) = d \}  E[  \ell (Y_{s},\theta) \mid D_{s}(x) = d ] = 1\{D_{s}(x) = d \}  E[  \ell (Y(d,x),\theta) ]$ as $Y(d,x)$ is IID and in particular independent of $D_{s}(x)$.  
%	
%	By Lemma \ref{lem:uniform.LLN}, for any $\gamma>0$,
%	\begin{align*}
%			\mathbf{P}  \left( \sup_{\theta \in \Theta}  \left| t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta)   \right| \geq r_{t} \right) \leq \gamma,
%	\end{align*}
%	where $r_{t} = \sqrt{1/(2C \gamma) }\sqrt{\Lambda(t,|\Theta|)} $ ($C$ is an universal constant defined inside the proof of the lemma).
%	
%	Henceforth, fix $\gamma$. The previous result implies that, with probability greater than $1-\gamma$, 
%	\begin{align*}
%		\int \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta)   \right\}   \mu^{o}_{0}(d,x)(d\theta) \leq   N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( E[ -  \ell (Y(d,x),\theta)  ] - \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv
%	\end{align*}
%	and
%	\begin{align*}
%		 \int \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta)   \right\}   \mu^{o}_{0}(d,x)(d\theta) 	\geq  N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( E[ -  \ell (Y(d,x),\theta)  ] + \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv.
%	\end{align*}
%	
%	Hence, since $KL_{d,x}(\theta) : = - E [  \ell (Y(d,x),\theta)  ]$ it follows that, with probability greater or equal to $1-\gamma$, 
%	\begin{align*}
%		\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq   \frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta) - \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta) + \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   } 
%		=  \frac{  \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta)   \leq v \right) e^{-N_{t}(d,x) v +  t r_{t}  } dv   } {  \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right) e^{-N_{t}(d,x)v  - t r_{t}  } dv   } .
%	\end{align*}
%
%
%%	One can also obtain a lower bound, which we mention for completeness as it is not needed to establish our result. Here it is:
%%	\begin{align*}
%%		\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq &  \frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta) + \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta) - \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   } \\
%%		= & \frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta)   \leq v \right) e^{-N_{t}(d,x)v - t r_{t} } dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)   \leq v \right) e^{-N_{t}(d,x)v + t r_{t} } dv   }  
%%	\end{align*}
%%	where the second line(s) follow from a change of variable. 
%\end{proof}


==> app_alpha.tex <==
\section{Properties of  $\alpha$}
\label{app:alpha}

\subsection{Proof of Proposition \ref{pro:alpha.asymptotics.general}}

%\begin{lemma}\label{lem:alpha.charac} 
%		For any $(d,x) \in \mathbb{D} \times \mathbb{X}$, any $o,o' \in \{0,...,L\}$ and any $\varepsilon>0$, with probability greater or equal than $1-v(t,\varepsilon) : = XXX$,
%\begin{align*}
%	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq  \frac{ N_{t}(d,x)  \int_{0}^{\infty} G_{o}(d,x)(u) \exp\{  -  N_{t}(d,x) u  \}    du   } { N_{t}(d,x)  \int_{0}^{\infty} G_{o'}(d,x)(u) \exp\{  - N_{t}(d,x) u  \}  du   }  \exp\{ 2t r(t, \varepsilon )   \}
%\end{align*}
%and
%\begin{align*}
%	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq  \frac{ N_{t}(d,x)  \int_{0}^{\infty} G_{o}(d,x)(u)   \exp\{  -  N_{t}(d,x) u  \}    du   } {N_{t}(d,x)   \int_{0}^{\infty}  G_{o'}(d,x)(u)  \exp\{  -  N_{t}(d,x) u  \}  du   }  \exp\{ -2t r(t, \varepsilon )   \}.
%\end{align*}
%with $r(t,\varepsilon ) : = XXXX$. 
%		
%\end{lemma}
%
%The characterization separates the role of the prior and the role of $t$ --- or more precisely, $N_{t}(d,x)$. It basically shows that, other than the error term given by $rXXX$, what matters for the behavior of the weights is the aforementioned function $G_{o}(d,x)$ at particular values of $u$, and the importance of each $u$ is determined by $u \mapsto N_{t}(d,x)  \exp\{  -  N_{t}(d,x) u  \}  $ which is an Exponential PDF with parameter $N_{t}(d,x)$.\footnote{An alternative interpretation is based on the fact that $\int_{0}^{\infty} G_{o}(d,x)(u) \exp\{  -  N_{t}(d,x) u  \}    du $ is the Laplace transform of $G_{o}(d,x)$ evaluated at $N_{t}(d,x)$.} Thus, as the number of observations for $(d,x)$ grows, this exponential PDF concentrates around $u=0$ thereby implying that the behavior of $	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   }$  is influenced by the ratio of $G_{o}(d,x)(u)/G_{o'}(d,x)(u)$ in a neighborhood of $0$. 

To show Proposition \ref{pro:alpha.asymptotics.general} we use the following lemmas whose proofs are relegated to the end of this appendix. The first lemma studies the process $g(Y_{s},D_{s},\theta) : = (1\{D_{s}(x) = d \} ( \ell (Y_{s},\theta)  - E[  \ell (Y_{s},\theta) \mid D_{s}(x)  ]  ) $ for all $s \geq 1$, where the expectation is taken with respect to $P$ and $\ell(.,\theta) : = \log p_{\theta}(.)/p(. \mid d,x )$ and $p(\cdot | d,x)$ is the true PDF of $Y(d,x)$. 

\begin{lemma}\label{lem:uniform.LLN} 
%	Suppose $\Theta \subseteq \mathbb{R}^{|\Theta|}$ is compact and there exists a $C < \infty$ and $\kappa > 0$ such that $$ \max_{\theta' \in \Theta} E[ \sup_{\theta \in B(\theta',\delta)  }  | \ell(Y(d,x),\theta) - \ell(Y(d,x),\theta') |^{2}  ] \leq C^{2} \delta^{2\kappa},~\forall \delta >0. $$
	Suppose $\Theta \subseteq \mathbb{R}^{|\Theta|}$ is compact and there exists a $\varphi : \mathbb{R}_{+} \rightarrow \mathbb{R}_{+}$ such that $\varphi(0)=0$ and increasing and $$ \max_{\theta' \in \Theta} E[ \sup_{\theta \in B(\theta',\delta)  }  | \ell(Y(d,x),\theta) - \ell(Y(d,x),\theta') |^{2}  ] \leq \varphi(\delta)^{2},~\forall \delta >0. $$
	 Then for any $t$ and $\gamma > 0$,  	
	\begin{align*}
		P\left( \sup_{\theta \in \Theta } |  t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta)  | \geq \sqrt{1/(2C \gamma) } \sqrt{ \Lambda(t, |\Theta|)  }  \right) \leq \gamma
	\end{align*} 
where $\Lambda(t,|\Theta|) : =  \min_{\delta \geq 0} ( t^{-1} \delta^{-|\Theta|} + \varphi(\delta)) $ and is decreasing in $t$ and increasing in $|\Theta|$ and $\lim_{t\rightarrow \infty} \Lambda(t,|\Theta|) = 0$.
\end{lemma}

The second lemma provides a non-asymptotic bound for the ratio of the weights for any two models. In particular, it relates the weights, $\alpha^{o}_{t}$, with the Laplace transformation of $$ u \mapsto G^{o}_{d,x}(u) : = \mu_{0}^{o}(d,x) (  KL_{d,x}(\theta) \leq u   ). $$ To ou knowledge, this result is new and might be of independent interest.

\begin{lemma}\label{lem:alpha.asymptotics.general}
		Take any $o,o' \in \{0,...,L\}$ and $(d,x) \in \mathbb{D}\times \mathbb{X}$. Suppose $\Theta \subseteq \mathbb{R}^{|\Theta|}$ is compact and there exists a $\varphi : \mathbb{R}_{+} \rightarrow \mathbb{R}_{+}$ such that $\varphi(0)=0$ and increasing and $$ \max_{\theta' \in \Theta} E[ \sup_{\theta \in B(\theta',\delta)  }  | \ell(Y(d,x),\theta) - \ell(Y(d,x),\theta') |^{2}  ] \leq \varphi(\delta)^{2},~\forall \delta >0. $$
		Then, for any $\gamma > 0$,
		\begin{align*}
			\frac{\alpha^{o}_{t}(d,x)}{\alpha^{o'}_{t}(d,x)} \leq \frac{ \int G^{o}_{d,x}(u)  e^{-N_{t}(d,x) u} du  }{ \int G^{o'}_{d,x}(u)  e^{-N_{t}(d,x) u} du } e^{t r_{t}}~\forall t,
		\end{align*}
		with probability larger than $1-\gamma$,  where $r_{t} : = O(\sqrt{1/\gamma } \sqrt{ \Lambda(t,|\Theta|)  }  )$. 
\end{lemma}




\begin{proof} [Proof of Proposition \ref{pro:alpha.asymptotics.general}] 
	
	Suppose the conditions in Lemmas \ref{lem:uniform.LLN} and  \ref{lem:alpha.asymptotics.general} hold (we show they do towards the end of the proof). In this case, it follows  that for any $\varepsilon>0$,
	\begin{align*}
		P_{\pi} \left( 	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq \varepsilon   \right) \leq P_{\pi} \left( 	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq \varepsilon  \cap S_{t}(\varepsilon ) \right) + P_{\pi} \left( S_{t}(\varepsilon )^{C}  \right)
	\end{align*}
	where $S_{t}(\varepsilon )$ is the set such that $N_{t}(d,x)/t  \geq e_{t}(d,x) - \varepsilon$ and $r^{-1}_{t} \sup_{\theta \in \Theta}  \left| t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta)   \right| \leq \varepsilon $. By Lemma \ref{lem:uniform.LLN}  and Lemma \ref{lem:concentration.freq}, $\lim_{t\rightarrow \infty} P_{\pi} (S_{t}(\varepsilon) ^{C} ) =0$. 
	
	In what follows, take an arbitrary sequence in $S_{t}(\varepsilon )$. Let $u_{o}(d,x)$ as in the definition. If $u_{o}(d,x) - u_{o'}(d,x) = : A > 0$, then by Lemma \ref{lem:alpha.asymptotics.general}, 
	\begin{align*}
		\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq & e^{2 t r_{t} }	\frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right) e^{-N_{t}(d,x)v} dv   } \\
		\leq & e^{2 t r_{t} }	\frac{ N_{t}(d,x) \int_{u_{o}(d,x)}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{u_{o'}(d,x)}^{ u_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)   \leq v \right) e^{-N_{t}(d,x)v} dv   }	\\
		\leq & e^{2 t r_{t} }	\frac{ e^{-N_{t}(d,x) u_{o}(d,x) }   \int_{u_{o}(d,x)}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x} (\theta)   \leq v \right) dv  } { e^{-N_{t}(d,x)  (  m_{o'}(d,x)  + 0.5 A )  } \int_{m_{o'}(d,x)}^{ u_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right)  dv   } \\
		= & e^{ - N_{t}(d,x)  0.5 A + 2 t r_{t}   }   \frac{  \int_{u_{o}(d,x)}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x} (\theta)   \leq v \right) dv  } {  \int_{u_{o'}(d,x)}^{ u_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right)  dv   }
	\end{align*}
	where the last line follows from definition of $A$. 
	
	The fraction in the previous display is a fixed number. Under the set $S_{t}(\varepsilon)$, $\frac{N_{t}(d,x)}{t}  0.5 A + 2 r_{t} \geq (e_{t}(d,x) - \varepsilon ) 0.5 A - 2 \varepsilon $. Under Assumption \ref{ass:PF.epsilon}, there exists a $\bar{\varepsilon}>0$ (not dependant on $t$) such that for any $\varepsilon \leq \bar{\varepsilon}$, $\frac{N_{t}(d,x)}{t}  0.5 A + 2 r_{t} \geq c > 0$. Thus, we obtain $\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } = O( e^{-t c } )$, which in turn implies that 
	\begin{align*}
		P_{\pi} \left( 	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq \varepsilon   \right) \leq P_{\pi} \left(  e^{-t c }  \geq \varepsilon  \right) + P_{\pi} \left( S_{t}(\varepsilon )^{C}  \right) = o(1),
	\end{align*}
	for any $\varepsilon \leq \bar{\varepsilon}$. Thus the desired result follows. 
	
	\bigskip
	
	We now verify that the conditions in Lemma \ref{lem:alpha.asymptotics.general} (and thus, Lemma \ref{lem:uniform.LLN}) hold. $\Theta$ is compact by assumption, so we ``just" need to verify the continuity condition. 
	
	By Assumption, $\theta \mapsto \log p_{\theta}(\cdot)$ is continuous a.s.-$P_{\pi}$. This implies that $\theta \mapsto \ell(\cdot,\theta)$ is continuous a.s.-$P_{\pi}$.  Continuous functions over compact sets are uniformly continuous, thus $f(Y(d,x),\delta) : = \sup_{||\theta-\theta'|| \leq \delta} |\ell(Y(d,x),\theta) - \ell(Y(d,x),\theta')| $ converges to 0 as $\delta$ vanishes a.s.-$P_{\pi}$. By Assumption, $E[\sup_{\theta \in \Theta} | \log p_{\theta} (Y(d,x))|^{2}   ] < \infty$, and thus by the Dominated convergence theorem, $\lim_{\delta \rightarrow 0} E[f(Y(d,x),\delta) ^{2} ] = 0$ as desired.  
	
	
	
	%
	%
	%If $\frac{t r_{t}}{N_{t}(d,x)} = o(1)$ XXX, then if follows that the RHS converges to to zero as $ e^{-N_{t}(d,x) m_{o}(d,x) } / e^{-N_{t}(d,x)  (  m_{o'}(d,x)  + 0.5 A )  }  = o(1)$ and $\int_{m_{o'}(d,x)}^{ m_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{o'}(d,x)(\theta) + \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right)  dv $ converges to $\int_{m_{o'}(d,x)}^{ m_{o'}(d,x)  + 0.5 A }  \mu^{o'}_{0}(d,x) \left( KL_{o'}(d,x)(\theta) \leq v \right)  dv >0 $.
	%
	%If $m_{o}(d,x) = m_{o'}(d,x) = A>0$ and $\frac{t r_{t}}{N_{t}(d,x)} = o(1)$, then
	%\begin{align*}
	%	& \frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{o}(d,x)(\theta) - \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{o'}(d,x)(\theta) + \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   }  \\
	%	\leq &  \frac{ N_{t}(d,x) \int_{A}^{\infty} G_{o}(d,x)(v) e^{-N_{t}(d,x)v} dv  + \left( \frac{t r_{t}}{N_{t}(d,x)} \right) ^{\rho} C e^{-N_{t}(d,x)A}  } { N_{t}(d,x) \int_{A}^{\infty}  G_{o'}(d,x) (v)  e^{-N_{t}(d,x)v} dv - \left( \frac{t r_{t}}{N_{t}(d,x)} \right) ^{\rho} C e^{-N_{t}(d,x)A}}.  
	%\end{align*}
	%
	%
	%
	%XXX Gaussian 
	%
	%Suppose $KL_{o}(d,x)(\theta) = 0.5(\theta(d,x) - \theta^{\ast}(d,x))^{2}$ and $\mu^{o}_{0}(d,x)$ is Gaussian with mean $\zeta_{0}^{o}(d,x)$ and $1/\nu_{0}^{o}(d,x)$. Then, for any $v \geq 0$, 
	%\begin{align*}
	%	 \mu^{o}_{0}(d,x) \left( KL_{o'}(d,x)(\theta)  \leq v \right) = & \int_{-\sqrt{2v} + \theta^{\ast}(d,x) }^{\sqrt{2v} + \theta^{\ast}(d,x) } \phi(w; \zeta_{0}^{o}(d,x), 1/\nu_{0}^{o}(d,x))dw \\
	%	 = & 2 \Phi( \sqrt{2v} + \theta^{\ast}(d,x) ; \zeta_{0}^{o}(d,x), 1/\nu_{0}^{o}(d,x) )
	%\end{align*}
	%
	%\begin{align*}
	%	\int_{0}^{\infty}  G_{o'}(d,x) (v)  e^{-N_{t}(d,x)v} dv  = \int_{A}^{\infty} 2 \Phi( \sqrt{2v} + \theta^{\ast}(d,x) ; \zeta_{0}^{o}(d,x), 1/\nu_{0}^{o}(d,x) )  e^{-N_{t}(d,x)v} dv  
	%\end{align*}
	%
	%
	%XXXXXXXXXXXXXXXXXXXXXXXXXX
	%
	%
	%Moreover XXXX. 
	%
	%Therefore, Lemma XXX implies that for any $\varepsilon>0$,
	%\begin{align*}
	%	P \left( \left| t^{-1} \sum_{s=1}^{t} g_{o}(Y_{s},D_{s},\theta)   \right| \geq r(t, \varepsilon ) \right) \leq v(t,\varepsilon)
	%\end{align*}
	%where $r(t,\varepsilon) : = XXX$ and $v(t,\varepsilon) : = XXX$. This result and the fact that $\sum_{s=1}^{t} 1\{D_{s} = d \} E [  \ell_{o} (Y_{s},\theta) \mid D_{s} ] = \sum_{s=1}^{t} 1\{D_{s} = d \} E [  \ell_{o} (Y_{s}(d),\theta)  ] = t f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ] $ imply that
	%	\begin{align*}
		%	P \left( \frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq \frac{\int \exp \left\{ t ( f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]  -  r(t, \varepsilon ) )  \right\}   \mu^{o}_{0}(d,x)(d\theta)} {\int \exp \left\{ t ( f_{t}(d) E [  \ell_{o'} (Y(d),\theta)  ]  + r(t, \varepsilon ) ) \right\} \mu^{o'}_{0}(d,x)(d\theta)   } \right) \geq 1 - v(t,\varepsilon) 
		%\end{align*}
		%and 
		%	\begin{align*}
			%	P \left( \frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq \frac{\int \exp \left\{ t ( f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]  +  r(t, \varepsilon ) )  \right\}   \mu^{o}_{0}(d,x)(d\theta)} {\int \exp \left\{ t ( f_{t}(d)  E [  \ell_{o'} (Y(d),\theta)  ]  - r(t, \varepsilon ) ) \right\} \mu^{o'}_{0}(d,x)(d\theta)   } \right) \geq 1 - v(t,\varepsilon) .
			%\end{align*}
			%
			%
			%Observe that
			% \begin{align*}
				%	\int \exp \{ t  f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]  \}  \mu^{o}_{0}(d,x)(d\theta) = & \int_{1}^{\infty} \mu^{o}_{0}(d,x) \left( \exp \{  t  f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ] \} \geq x     \right) dx \\
				%	= & \int_{1}^{\infty} \mu^{o}_{0}(d,x) \left(   t  f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]  \geq (\log x)/(  t  f_{t}(d)  )      \right) dx \\
				%	= & t f_{t}(d)  \int_{0}^{\infty} \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  f_{t}(d) u  \} du  
				%\end{align*}
				%where the 3rd equality follows from a change of variables $u = (\log x)/(  t  f_{t}(d)  )$ where 
				% $ t f_{t}(d) \exp\{  t  f_{t}(d) u  \} du = dx $. Thus,
				%\begin{align*}
				%	\frac{\int \exp \left\{ t  f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]   \right\}   \mu^{o}_{0}(d,x)(d\theta)} {\int \exp \left\{ t f_{t}(d)  E [  \ell_{o'} (Y(d),\theta)  ]  \right\} \mu^{o'}_{0}(d,x)(d\theta)   } = \frac{ \int_{0}^{\infty} \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  f_{t}(d) u  \}    du   } {  \int_{0}^{\infty} \mu^{o'}_{0}(d,x) \left(   E [  \ell_{o'} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  f_{t}(d) u  \}  du   }  .
				%\end{align*}
				%
				%Hence, since $KL_{o}(d,x)(\theta) : = - E [  \ell_{o} (Y(d),\theta)  ]$ it follows that, with probability greater or equal to $1-v(\varepsilon,t)$,
				%
				%%\begin{align*}
				%%	 \frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq  \frac{ \int_{0}^{\infty} \mu^{o}_{0}(d,x) \left(   KL_{o}(d,x)(\theta)  \leq -u   \right)  \exp\{  t  f_{t}(d) u  \}    du   } {  \int_{0}^{\infty} \mu^{o'}_{0}(d,x) \left(   KL_{o'}(d,x)(\theta) \leq -u   \right)  \exp\{  t  f_{t}(d) u  \}  du   }  \exp\{ 2t r(t, \varepsilon )   \}
				%%\end{align*}
				%\begin{align*}
				%	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq  \frac{ \int_{0}^{\infty} \mu^{o}_{0}(d,x) \left(   KL_{o}(d,x)(\theta)  \leq u   \right)  \exp\{  -t  f_{t}(d) u  \}    du   } {  \int_{0}^{\infty} \mu^{o'}_{0}(d,x) \left(   KL_{o'}(d,x)(\theta) \leq u   \right)  \exp\{  -t  f_{t}(d) u  \}  du   }  \exp\{ 2t r(t, \varepsilon )   \}
				%\end{align*}
				%and
				%\begin{align*}
				%	\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq  \frac{ \int_{0}^{\infty} \mu^{o}_{0}(d,x) \left(  KL_{o}(d,x)(\theta)  \leq u   \right)  \exp\{  - t  f_{t}(d) u  \}    du   } {  \int_{0}^{\infty} \mu^{o'}_{0}(d,x) \left(   KL_{o'}(d,x)(\theta) \leq u   \right)  \exp\{  - t  f_{t}(d) u  \}  du   }  \exp\{ -2t r(t, \varepsilon )   \}.
				%\end{align*}
				%
				%$u \mapsto \mu^{o}_{0}(d,x) \left(   KL_{o}(d,x)(\theta)  \leq u   \right)  = : G_{o}(d,x)(u)$ is a CDF. 
				
				%
				%XXXXXXXXXXXXXXXXXXXXXXXXXXXXX
				%
				%
				%XXXXX
				%
				%If support are different: 
				%
				%\begin{align*}
				%	\frac{\int \exp \left\{ t  f_{t}(d) E [  \ell_{o} (Y(d),\theta)  ]   \right\}   \mu^{o}_{0}(d,x)(d\theta)} {\int \exp \left\{ t f_{t}(d)  E [  \ell_{o'} (Y_{s}(d),\theta)  ]  \right\} \mu^{o'}_{0}(d,x)(d\theta)   } \leq & \frac{ \int_{0}^{A} \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  f_{t}(d) u  \}    du   } {  \int_{A+\delta}^{B} \mu^{o'}_{0}(d,x) \left(   E [  \ell_{o'} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  f_{t}(d) u  \}  du   }  \\
				%	\leq &  \frac{  \exp\{  t  f_{t}(d) A  \}   \int_{0}^{A} \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq u   \right)   du   } {  \exp\{  t  f_{t}(d) (A + \delta)  \}    \int_{A+\delta}^{B} \mu^{o'}_{0}(d,x) \left(   E [  \ell_{o'} (Y(d),\theta)  ]  \geq u   \right)  du   } 
				%\end{align*}
				%
				%If support are the same:
				%
				%\begin{align*}
				%& \frac{ \int_{0}^{A} \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t  ( f_{t}(d) u  + r(t,\epsilon) )  \}    du   } {  \int_{0}^{A} \mu^{o'}_{0}(d,x) \left(   E [  \ell_{o'} (Y(d),\theta)  ]  \geq u   \right)  \exp\{  t ( f_{t}(d) u  - r(t,\epsilon) )   \}  du   }  \\
				%= & \frac{ \int_{0}^{  t(  r(t,\epsilon)  + A f_{t}(d))  } \mu^{o}_{0}(d,x) \left(   E [  \ell_{o} (Y(d),\theta)  ]  \geq (v/t  - r(t,\epsilon) )/ f_{t}(d)   \right)  \exp\{  v   \}    dv  } {  \int_{0}^{ t ( - r(t,\epsilon)  + A f_{t}(d) ) } \mu^{o'}_{0}(d,x) \left(   E [  \ell_{o'} (Y(d),\theta)  ]  \geq (v/t  + r(t,\epsilon) )/ f_{t}(d)   \right)  \exp\{  v   \}  dv   } 
				%\end{align*}
				%
				%
				%XXXXXXXXXXXXX
				%
				%Moreover, 
				%\begin{align*}
				%	\int \exp \left\{ t ( f_{t}(d) E [  \ell_{o} (Y_{s}(d),\theta)  ]  +  r(t, \epsilon ) )  \right\}   \mu^{o}_{0}(d,x)(d\theta) \leq \exp \left\{ t ( f_{t}(d) \max_{\theta \in \Theta_{o}}   E [  \ell_{o} (Y_{s}(d),\theta)  ]  +  r(t, \epsilon ) )  \right\}
				%\end{align*}
				%and
				%\begin{align*}
				%	\int \exp \left\{ t ( f_{t}(d) E [  \ell_{o} (Y_{s}(d),\theta)  ]  +  r(t, \epsilon ) )  \right\}   \mu^{o}_{0}(d,x)(d\theta) \geq \exp \left\{ t ( f_{t}(d) \min_{\theta \in \Theta_{o}(\delta)  }   E [  \ell_{o} (Y_{s}(d),\theta)  ]  +  r(t, \epsilon ) )  \right\} \mu_{0}^{o}( \Theta_{o}(\delta)  )
				%\end{align*}
				% where, for any $\delta> 0$, $\Theta_{o}(\delta)  : = \{ \theta \in \Theta_{o} \colon E [  \ell_{o} (Y_{s}(d),\theta)  ]  \geq  \max_{\theta \in \Theta_{o}}   E [  \ell_{o} (Y_{s}(d),\theta)  ]  - \delta     \}$.
				% 
				% XXXXXXX
				% 
			\end{proof}
			

\subsection{Proof of Lemma  \ref{lem:alpha.properties} }

\begin{proof}[Proof of Lemma \ref{lem:alpha.properties} ]
	Let $p_{\theta}$ denote a Gaussian PDF with mean $\theta$ and variance $1$. 
	
	(1) It follows that 
	\begin{align*}
		& \int \prod_{s=1}^{t} ( p_{\theta}(Y_{s}) )^{1\{ D_{s}(x) =d  \}}  \mu^{o}_{0}(d,x)(d\theta) \\
		= & \int (2\pi)^{-0.5 \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \} }\exp \left\{ - \frac{1}{2} \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \} \left( Y_{s} - \theta    \right)^{2}   \right\} \phi(\theta; \zeta^{o}_{0}(d,x) , 1/\nu_{0}^{o}(d,x) ) d\theta\\
		= & \int (2\pi)^{-0.5 \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \}   }\exp \left\{ - \frac{1}{2} \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \} \left( Y_{s}(d,x) - m_{t}(d,x)    \right)^{2}   \right\}\\
		\times & \exp \left\{ - \frac{1}{2} \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \} \left( m_{t}(d,x) - \theta    \right)^{2}   \right\} \\
		\times & \exp \left\{ - \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \} \left( Y_{s}(d,x) - m_{t}(d,x)    \right) \left( m_{t}(d,x) - \theta    \right)   \right\} \\	
		&  \phi(\theta; \zeta^{o}_{0}(d,x) , 1/\nu_{0}^{o}(d,x) ) d\theta,
	\end{align*}
	where $m_{t}(d,x) : = \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \}  Y_{s}(d,x) /\sum_{s=1}^{t} 1\{ D_{s}(x) =d  \}$. Observe that 
	\begin{align*}
		\sum_{s=1}^{t} 1\{ D_{s}(x) =d  \} \left( Y_{s}(d,x) - m_{t}(d,x)    \right) =  0 , 
	\end{align*}
	so, letting $N_{t}(d,x) : = \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \}$ it follows that 
	\begin{align*}
		\int 	\prod_{s=1}^{t} ( p_{\theta}(Y_{s}) )^{1\{ D_{s}(x) =d  \}}  \mu^{o}_{0}(d,x)(d\theta) = & (2\pi)^{-0.5 \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \} + 0.5}  N_{t}(d,x)^{-1/2}\\
		& \times  \exp \left\{ - \frac{1}{2} \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \} \left( Y_{s}(d,x) - m_{t}(d,x)    \right)^{2}   \right\}\\
		\times & \int (2\pi/N_{t}(d,x))^{-1/2} \exp \left\{ - \frac{1}{2}  \left( m_{t}(d,x) - \theta    \right)^{2} N_{t}(d,x)   \right\} \\	
		&  \phi(\theta; \zeta^{o}_{0}(d,x) , 1/\nu_{0}^{o}(d,x) ) d\theta.
	\end{align*}
	
	The expression of the integral can be viewed as a convolution between to Gaussian PDFs one indexed by $(  0,   1/N_{t}(d,x) )$ and $(  \zeta^{o}_{0}(d,x) , 1/\nu_{0}^{o}(d,x)  )$ resp, which in turn is equivalent to PDF of the sum of the corresponding random variables evaluated at $m_{t}(d,x)$. Therefore, 
	\begin{align*}
		\int \prod_{s=1}^{t} ( p_{\theta}(Y_{s}) )^{1\{ D_{s}(x) =d  \}}  \mu^{o}_{0}(d,x)(d\theta)  = C \phi( m_{t}(d,x) ; \zeta^{o}_{0}(d,x) , ( N_{t}(d,x)  + \nu^{o}_{0}(d,x)  )/( N_{t}(d,x)\nu^{o}_{0}(d,x) ) )
	\end{align*}
	where $C : = (2\pi)^{-0.5 \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \} + 0.5}   N_{t}(d,x)^{-1/2} \exp \left\{ - \frac{1}{2} \sum_{s=1}^{t} 1\{ D_{s}(x) =d  \} \left( Y_{s}(d,x) - m_{t}(d,x)    \right)^{2}   \right\}$ which, importantly, doesn't depend on the model $o$. 
	
	Hence
	\begin{align*}
		\alpha^{o}_{t}(d,x) = \frac{       \phi( m_{t}(d,x) ; \zeta^{o}_{0}(d,x) , ( N_{t}(d,x)  + \nu^{o}_{0}(d,x)  )/( N_{t}(d,x)\nu^{o}_{0}(d,x) ) )       }  {  \sum_{o=0}^{L}   \phi( m_{t}(d,x) ; \zeta^{o}_{0}(d,x) , ( N_{t}(d,x)  + \nu^{o}_{0}(d,x)  )/( N_{t}(d,x)\nu^{o}_{0}(d,x) ) )    }  
	\end{align*} 
	
	
	(2) Follows from the definition of $\phi$. \\
	
	(3) By Lemmas \ref{lem:concentration.freq} and \ref{lem:concentration.avg} and Assumption \ref{ass:PF.epsilon}, $N_{t}(d,x)$ diverges with probability approaching 1 and $m_{t}(d,x) = \theta(d,x) + o_{P}(1)$. By continuity of $\phi$, the result follows. 
\end{proof}

\subsection{Bounds for $\alpha_{t}$} 


It follows that, tor any $(d,x) \in \mathbb{D}\times \mathbb{X}$ and $t$,   $\alpha^{o}_{t}(d,x) =  \frac{   \exp  \ell^{o}_{t}(d,x)   }   {    \sum_{o=0}^{L}  \exp  \ell^{o}_{t}(d,x)      }   $ where 
\begin{align*}
	\ell^{o}_{t}(d,x)  : =  \log \phi  (m_{t}(d,x)   ;  \zeta^{o}_{0}(d,x) ,   ( N_{t}(d,x) + \nu^{o}_{0}(d,x)  )/(N_{t}(d,x)\nu^{o}_{0}(d,x) )    ) 
\end{align*}
We now provide non-random bounds for  $\ell^{o}_{t}$ and study some properties; all proofs are relegated to the end of the section. Finally, recall that $f_{t}(d,x) : = N_{t}(d,x) / t$. 




\begin{lemma}\label{lem:alpha.bound} 
	For any $o \in \{ 0,...,L  \}$, any $(d,x) \in \mathbb{D}\times \mathbb{X}$, any $\pi_{t}(d,x) \in (0,1)$ and $\eta \in (0,\epsilon)$, $\delta > 0$ such that $| f_{t}(d,x)  - \pi_{t}(d,x)| \leq \eta$ and $| m_{t}(d,x) - \theta (d,x)| \leq \delta$, it follows that 
	\begin{align*}
	\underline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x)| , \nu^{o}_{0}(d,x) , \pi_{t}(d,x)  ) \leq	\ell^{o}_{t}(d,x) \leq   \overline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x)  ), 
	\end{align*} 
and thus
\begin{align*}
	\underline{\alpha}^{o}(  \eta ,\delta , |\bar{\zeta}_{0}(d,x) | ,  \nu_{0}(d,x) , \pi_{t}(d,x)  )    \leq  \alpha^{o}_{t}(d,x)  \leq   	\overline{\alpha}^{o}( \eta ,\delta,  |\bar{\zeta}_{0}(d,x) | ,  \nu_{0}(d,x) , \pi_{t}(d,x)  )
\end{align*}
where 
\begin{align*}
	\underline{\alpha}^{o}( \eta ,\delta, |\bar{\zeta}_{0}(d,x) | ,  \nu_{0}(d,x) , \pi_{t}(d,x)  )  : = 	\frac{  e^{  \underline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | ,  \nu^{o}_{0}(d,x) , \pi_{t}(d,x)   )}   }   {    \sum_{o=0}^{L}  e^{ \overline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | ,  \nu^{o}_{0}(d,x) , \pi_{t}(d,x)   )  }   }    
\end{align*}
and 
\begin{align*}
	\overline{\alpha}^{o}( \delta,  \eta,  |\bar{\zeta}_{0}(d,x) | ,  \nu_{0}(d,x) , \pi_{t}(d,x)  )	: = \frac{  e^{  \overline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x) | ,  \nu^{o}_{0}(d,x) , \pi_{t}(d,x)   ) } }   {    \sum_{o=0}^{L}  e^{ \underline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x) | ,  \nu^{o}_{0}(d,x) , \pi_{t}(d,x)  ) }     },  
\end{align*}
and
	\begin{align*}
\overline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x) | ,  \nu^{o}_{0}(d,x) , \pi_{t}(d,x)   ) : = - \log  \underline{\sigma}_{t}(d,x)   - 0.5 \frac{   ( \delta -  |\bar{\zeta}^{o}_{0}(d,x) |  ) ^{2}     }{   \overline{\sigma}^{2}_{t}(d,x)   } ,
	\end{align*}
%		\begin{align*}
%\underline{\ell}( \delta, \eta , |\bar{\zeta}^{o}_{0}(d,x) | ,  \nu^{o}_{0}(d,x) , \pi_{t}(d,x)   ) : = \min\{  \log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \overline{\sigma}^{2}_{t}(d,x))    ,   	\log  \phi( \delta  ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \underline{\sigma}^{2}_{t}(d,x))    \} ,
%\end{align*} 
\begin{align*}
	\underline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) ,  \pi_{t}(d,x)  ) : =  & 1\{ (\delta + |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} < \overline{\sigma}^{2}_{t}(d,x) \}     \log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \overline{\sigma}^{2}_{t}(d,x))    \\
	& +    1\{ (\delta + |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} > \underline{\sigma}^{2}_{t}(d,x) \} 	\log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \underline{\sigma}^{2}_{t}(d,x))    \} .
\end{align*}

and
\begin{align*}
	& \sigma^{2}_{t}(d,x)  \geq 	\underline{\sigma}^{2}_{t}(d,x) : = 1/\nu^{o}_{0}(d,x) + t^{-1} /(\pi_{t}(d,x) + \eta)  \\
	  ~and~ &	\sigma^{2}_{t}(d,x)  \leq 	\overline{\sigma}^{2}_{t}(d,x) : = 1/\nu^{o}_{0}(d,x) + t^{-1} /(\pi_{t}(d,x) - \eta)  .
\end{align*} 
\end{lemma}

\begin{remark}
  For any $\eta \in (0,\epsilon)$, we define  $$\overline{\ell}( \eta , |\bar{\zeta}^{o}_{0}(d,x) | ,  \nu^{o}_{0}(d,x) , \pi_{t}(d,x)   )  : =  \overline{\ell}( \eta, \eta , |\bar{\zeta}^{o}_{0}(d,x) | ,  \nu^{o}_{0}(d,x) , \pi_{t}(d,x)   )$$ and $$\underline{\ell}( \eta , |\bar{\zeta}^{o}_{0}(d,x) | ,  \nu^{o}_{0}(d,x) , \pi_{t}(d,x)   )  : = \underline{\ell}( \eta, \eta , |\bar{\zeta}^{o}_{0}(d,x) | ,  \nu^{o}_{0}(d,x) , \pi_{t}(d,x)   ).  $$ $\triangle$ 
\end{remark}



The next lemma summarizes some useful properties of $\underline{\ell}$ and $\overline{\ell}$.

\begin{lemma}\label{lem:ell.properties}
	The following propertis are true:
	\begin{enumerate}
	%	\item $a \mapsto \overline{\ell}( \eta , a, \nu^{o}_{0}(d,x) , \pi_{t}(d,x)  ) $ and $a \mapsto \underline{\ell}( \eta , a, \nu^{o}_{0}(d,x) , \pi_{t}(d,x)  ) $ are decreasing. 
		\item As $|\bar{\zeta}^{o}_{0}(d,x) | \rightarrow \infty$, $\overline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x)  )$ and $\underline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x) )$ converge to $-\infty$.
		
		\item $\eta \mapsto \overline{\ell}( \eta ,\delta  , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x)  )$  is increasing and $\eta \mapsto \overline{\ell}( \eta ,\delta  , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x)  )$ is decreasing.
		
%		\item Over the set $\{ \delta :  \delta < |\bar{\zeta}^{o}_{0}(d,x) |\}$, $\delta \mapsto \overline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x) )$ is increasing and over the set $\{ \delta :  \delta > |\bar{\zeta}^{o}_{0}(d,x) |\}$, $\delta \mapsto \overline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x) )$ is decreasing. Also, $\delta \mapsto \underline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x) )$ is decreasing.
\item $\delta \mapsto \overline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x) )$ is non-decreasing, and $\delta \mapsto \underline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x) )$ is decreasing.
		
		
		\item Suppose Assumption \ref{ass:PF.epsilon} holds and $\pi_{t} = e_{t}$. For any $\eta < \epsilon$, $\underline{\sigma}^{2}_{t}(d,x) \geq 1/\nu^{o}_{0}(d,x) + t^{-1}/(1 + \eta)  = : \dot{\underline{\sigma}}^{2}_{t}(d,x) $ and $\overline{\sigma}^{2}_{t}(d,x) \leq 1/\nu^{o}_{0}(d,x) + t^{-1}/(\epsilon - \eta) = : \dot{\overline{\sigma}}^{2}_{t}(d,x) $. Thus, 
		\begin{align*}
			\overline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x)  ) \leq   \overline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) )
		\end{align*}
	and
			\begin{align*}
		\underline{\ell}( \eta ,\delta  , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x)  ) \geq   \underline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) )
	\end{align*}
	where the RHS bounds are defined as $	\overline{\ell}$ and $\overline{\ell}$ but using $ \dot{\overline{\sigma}}$ and $ \dot{\underline{\sigma}}$ instead of $\overline{\sigma}$ and $\underline{\sigma}$. The usefulness of these bounds is that they do not depend on $e_{t}$ but they still inherit properties 1-3.
	
	Moreover, 
	\begin{align*}
		\underline{\alpha}^{o}( \eta ,\delta ,  |\bar{\zeta}_{0}(d,x) | , \nu_{0}(d,x) , e_{t}(d,x) ) \geq \underline{\alpha}^{o}( \eta ,\delta,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x)  )  : = \frac{ e^{ \underline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) ) }  }{ \sum_{o'=0}^{L} e^{\overline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) )}   } 
	\end{align*}
	and
		\begin{align*}
		\overline{\alpha}^{o}( \eta ,\delta,  |\bar{\zeta}_{0}(d,x) | , \nu_{0}(d,x) , e_{t}(d,x) ) \geq \overline{\alpha}^{o}( \eta ,\delta, |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x)  )  : = \frac{ e^{ \overline{\ell}( \eta ,\delta  , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) ) }  }{ \sum_{o'=0}^{L} e^{\underline{\ell}( \eta ,\delta , |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) ) }  } .
	\end{align*}
	
	\item The functions	$\overline{\alpha}^{o}( \eta ,\delta,  |\bar{\zeta}_{0}(d,x) | , \nu_{0}(d,x) , e_{t}(d,x) ) $ and $\overline{\alpha}^{o}( \eta ,\delta, |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x)  ) $ are increasing in $\eta$ and $\delta$. 
	
%		\item Suppose $|\bar{\zeta}^{o}_{0}(d,x) | = 0$. Then 
%		\begin{align*}
%		&	\lim_{  \nu^{o}_{0}(d,x) \rightarrow \infty  }  \overline{\ell}( \delta, \eta ,0, \nu^{o}_{0}(d,x) , \pi_{t}(d,x)  ) = \log ( t ( \pi_{t}(d,x) + \eta) ) ,\\
%		&	\lim_{  \nu^{o}_{0}(d,x) \rightarrow \infty  }  \underline{\ell}( \delta, \eta ,0, \nu^{o}_{0}(d,x)  ,  \pi_{t}(d,x) ) = \min \{ \log \phi(  \eta; 0, 1/((\pi_{t}(d,x) - \eta  )   ) , \log \phi(  \eta; 0, 1/((\pi_{t}(d,x) + \eta  )   )  )   \}	.
%			\end{align*}
	\end{enumerate}
\end{lemma}

Property 1 is key for our analysis. It shows that the upper and lower bound maintain a key property of the weights: If the bias of a model is ``very large", then the corresponding weight will be ``small". 



\subsection{Proof of Supplemental Lemmas}

\begin{proof}[Proof of Lemma \ref{lem:uniform.LLN} ]	
	Henceforth, we omit the notation "$x$" from the quantities as there is no risk of confusion. Let $\mathcal{F}^{s}$ denote the $\sigma$-algebra generated by $(D_{1},...,D_{s},Y_{1},...,Y_{s-1})$. We now show that for each $\theta \in \Theta$, $(g(Y_{s},D_{s},\theta))_{s}$ is a MDS with respect to aforementioned $\sigma$-algebras. To do this, note that 
	\begin{align*}
		E[ g(Y_{s},D_{s},\theta) \mid  \mathcal{F}^{s} ] = 1\{D_{s} = d \}  E[ \ell (Y_{s},\theta)  - E[  \ell (Y_{s},\theta) \mid D_{s} ] \mid  \mathcal{F}^{s} ].
	\end{align*}
	Observe that $E[ \ell (Y_{s},\theta)  \mid  \mathcal{F}^{s} ] = E[ \ell (Y_{s},\theta)  \mid  D_{s} ] $ because $Y_{s}$ is independent of the whole past once we condition on $D_{s}$. Since $E[[  \ell (Y_{s},\theta) \mid D_{s} ] \mid  \mathcal{F}^{s} ] = E [  \ell (Y_{s},\theta) \mid D_{s} ] $, it follows that $E[ g(Y_{s},D_{s},\theta) \mid  \mathcal{F}^{s} ]  = 0$. 
	
	
	Since $\Theta$ is assumed to be compact, for any $\delta>0$, there exists a $L_{\delta}$ such that $\Theta \subseteq \cup_{l =1}^{L} B(\theta_{l},\delta)$ where $B(\theta,\delta)$ is a $\delta$-radius ball with center $\theta$. Indeed, let $L_{\delta}$ be the smallest number of balls of radius $\delta$ needed to cover the set, and as $\Theta \subseteq \mathbb{R}^{|\Theta|}$, it follows that $L_{\delta} \leq C \delta^{-|\Theta|}$ where $C$ is an universal constant. %; see XXX. 
	Thus, for any $t$ and any $\delta>0$,
	\begin{align*}
		\sup_{\theta \in \Theta}  |t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta) | \leq &	\max_{l \in \{1,...,L_{\delta} \}}  |t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta_{l}) |  \\
		& +  	\max_{l \in \{1,...,L_{\delta} \}}  	\sup_{\theta \in B(\theta_{l},\delta)  }  |t^{-1} \sum_{s=1}^{t} \{  g(Y_{s},D_{s},\theta) - g(Y_{s},D_{s},\theta_{l})\} | .
	\end{align*}
	
	%	We now show that for any $\varepsilon$, there exists a $\delta$ (not dependening on $t$ nor $l$) such that $$E[ \sup_{\theta \in B(\theta_{l},\delta)  }  |t^{-1} \sum_{s=1}^{t} \{  g_{o}(Y_{s},D_{s},\theta) - g_{o}(Y_{s},D_{s},\theta_{l})\} | ]  \leq  \varepsilon .$$ This follows because, by assumption XXX, 
	By the triangle inequality and simple algebra, for any $t$, any $\delta>0$ and any $l \in \{1,...,L_{\delta}\}$,
	\begin{align*}
		& \sqrt{E[ \sup_{\theta \in B(\theta_{l},\delta)  }  |t^{-1} \sum_{s=1}^{t} \{  g(Y_{s},D_{s},\theta) - g(Y_{s},D_{s},\theta_{l})\} |^{2}  ] } \\
		\leq & t^{-1} \sum_{s=1}^{t} \sqrt{E[ \sup_{\theta \in B(\theta_{l},\delta)  }  | g(Y_{s},D_{s},\theta) - g(Y_{s},D_{s},\theta_{l}) |^{2}  ] }\\
		\leq & 2 t^{-1} \sum_{s=1}^{t } \sqrt{E[ \sup_{\theta \in B(\theta_{l},\delta)  }  | \ell(Y_{s}(d,x),\theta) - \ell(Y_{s}(d,x),\theta_{l})) |^{2}  ] } \\
		\leq & 2 \sqrt{E[ \sup_{\theta \in B(\theta_{l},\delta)  }  | \ell(Y(d,x),\theta) - \ell(Y(d,x),\theta_{l})) |^{2}  ]} 			 
	\end{align*}
	where the last line follows from IID-ness of $Y(d,x)$. By Assumption, the RHS is less than $\varphi( \delta ) $. 
	
	By the Martingale difference property, for any $t$ and any $\delta>0$, 
	\begin{align*}
		E[( 	\max_{l \in \{1,...,L_{\delta} \}}  |t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta_{l}) |  )^{2} ] \leq & L_{\delta} t^{-1} \max_{1 \leq s \leq t} E[(  g(Y_{s},D_{s},\theta_{l})  )^{2} ] \leq C L_{\delta} t^{-1} \max_{1 \leq s \leq t} E[(  \ell(Y(d,x),\theta_{l})  )^{2} ]
	\end{align*} 
	for some universal constant $C$. Since $\Theta$ is bounded, the continuity assumption implies that $\max_{l} E[(  \ell(Y(d,x),\theta_{l})  )^{2} ] \leq C$ for some finite constant. 
	
	Then, by the Markov inequality, for any $\varepsilon>0$, any $t$ and any $\delta>0$,
	\begin{align*}
		P\left( \sup_{\theta \in \Theta } |  t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta)  | \geq \varepsilon   \right) \leq & C ( \varepsilon^{-2} t^{-1} L_{\delta} +  \varepsilon^{-1} \varphi( \delta )  ) \leq C \varepsilon^{-2} (  t^{-1} \delta^{-|\Theta|} +  \varphi( \delta )   ) 
	\end{align*}
	
	For any $t$, choose $\delta$ as the argmin of $\Lambda(t,|\Theta|) : =  \min_{\delta \geq 0} ( t^{-1} \delta^{-|\Theta|} + \varphi(\delta)) $. %This implies that $  t^{-1} \delta^{-|\Theta|} +  \delta^{\kappa} = 2 t^{-\frac{\kappa}{ |\Theta| + \kappa }}$. 
	Observe that $\Lambda(.,.)$ is decreasing in $t$ and increasing in $|\Theta|$ and $\lim_{t\rightarrow \infty} \Lambda(t,|\Theta|) = 0$; the first property is straightforward and the second one follows because $t^{-1} \delta^{-|\Theta|} + \varphi(\delta)$ converges to $\varphi(\delta)$ (pointwise) and $\varphi(0) = 0$. 
	
	
	Hence, by choosing $\varepsilon = \sqrt{(0.5/C) M} \sqrt{ \Lambda(t,|\Theta|)  } $ for any $M>0$ it follows that
	\begin{align*}
		P\left( \sup_{\theta \in \Theta } |  t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta)  | \geq \sqrt{(0.5/C) M} \sqrt{ \Lambda(t,|\Theta|)  }    \right) \leq & C ( \varepsilon^{-2} t^{-1} L_{\delta} +  \varepsilon^{-1}  \delta^{\kappa}) \leq M^{-1} 
	\end{align*} 
	for any $t$. Thus, $r_{t} : = \sqrt{(0.5/C) M} \sqrt{ \Lambda(t,|\Theta|)  } $ and re-defining $M$ as $1/\gamma$ the desired result follows. 
	
\end{proof}

\begin{proof} [Proof of Lemma  \ref{lem:alpha.asymptotics.general}] 
	For any $(d,x) \in \mathbb{D} \times \mathbb{X}$ and any $o,o' \in \{0,...,L\}$ observe that 
	\begin{align*}
		\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } = \frac{\int \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta)  \right\}   \mu^{o}_{0}(d,x)(d\theta)} {\int \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell(Y_{s},\theta)  \right\} \mu^{o'}_{0}(d,x)(d\theta)   }
	\end{align*}
	where $\ell(.,\theta) : = \log p_{\theta}(.)/p(. \mid d,x )$ and $p(\cdot | d,x)$ is the true PDF of $Y(d,x)$. 
	
	We observe that 
	\begin{align*}
		& \int \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta)   \right\}   \mu^{o}_{0}(d,x)(d\theta) \\
		= & \int_{1}^{\infty}  \mu^{o}_{0}(d,x) \left(  \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta)  \right\} \geq u \right) du \\
		= & N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( - N^{-1}_{t}(d,x)  \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta)  \leq v \right) e^{-N_{t}(d,x)v} dv
	\end{align*}
	where the second equality is obtained by a change of variables $v = - N^{-1}_{t}(d,x) \log u$. 
	
	In addition, note that
	\begin{align*}
		N^{-1}_{t}(d,x)  \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta) = & \frac{t}{N_{t}(d,x)} t^{-1}  \sum_{s=1}^{t}  g(Y_{s},D_{s},\theta) \\
		& + 	N^{-1}_{t}(d,x)  \sum_{s=1}^{t} 1\{D_{s}(x) = d \} E[  \ell (Y_{s},\theta) \mid D_{s}  ] \\
		= & \frac{t}{N_{t}(d,x)} t^{-1}  \sum_{s=1}^{t}  g(Y_{s},D_{s},\theta)  + E[  \ell (Y(d,x),\theta)  ] 
	\end{align*}
	where $g(Y_{s},D_{s},\theta) : = (1\{D_{s}(x) = d \} ( \ell (Y_{s},\theta)  - E[  \ell (Y_{s},\theta) \mid D_{s}(x)  ]  ) $  and the last line follows because $1\{D_{s}(x) = d \} E[  \ell (Y_{s},\theta) \mid D_{s}(x)  ] = E[  \ell (Y_{s},\theta) \mid D_{s}(x) = d ] = E[  \ell (Y_{s}(d,x),\theta) ]$ as $Y(d,x)$ is IID and in particular independent of $D_{s}(x)$.  
	
	By Lemma \ref{lem:uniform.LLN}, for any $\gamma>0$,
	\begin{align*}
		P \left( \sup_{\theta \in \Theta}  \left| t^{-1} \sum_{s=1}^{t} g(Y_{s},D_{s},\theta)   \right| \geq r_{t} \right) \leq \gamma,
	\end{align*}
	where $r_{t} = \sqrt{1/(2C \gamma) } t^{-0.5\frac{\kappa}{ |\Theta| + \kappa }} $ ($C$ is an universal constant defined inside the proof of the lemma).
	
	Henceforth, fix $\gamma$. The previous result implies that, with probability greater than $1-\gamma$, 
	\begin{align*}
		& \int \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta)   \right\}   \mu^{o}_{0}(d,x)(d\theta) \\
		\leq &  N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( E[ -  \ell (Y(d,x),\theta)  ] - \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv
	\end{align*}
	and
	\begin{align*}
		& \int \exp \left\{ \sum_{s=1}^{t} 1\{D_{s}(x) = d \} \ell (Y_{s},\theta)   \right\}   \mu^{o}_{0}(d,x)(d\theta) \\
		\geq &  N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( E[ -  \ell (Y(d,x),\theta)  ] + \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv.
	\end{align*}
	
	Hence, since $KL_{d,x}(\theta) : = - E [  \ell (Y(d,x),\theta)  ]$ it follows that, with probability greater or equal to $1-\gamma$, 
	\begin{align*}
		\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \leq &  \frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta) - \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta) + \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   } \\
		= & \frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta)   \leq v \right) e^{-N_{t}(d,x) v +  t r_{t}  } dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)  \leq v \right) e^{-N_{t}(d,x)v  - t r_{t}  } dv   } 
	\end{align*}
	and
	\begin{align*}
		\frac{\alpha^{o}_{t}(d,x) }{ \alpha^{o'}_{t}(d,x)   } \geq &  \frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta) + \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta) - \frac{t r_{t}}{N_{t}(d,x)}  \leq v \right) e^{-N_{t}(d,x)v} dv   } \\
		= & \frac{ N_{t}(d,x) \int_{0}^{\infty}  \mu^{o}_{0}(d,x) \left( KL_{d,x}(\theta)   \leq v \right) e^{-N_{t}(d,x)v - t r_{t} } dv   } { N_{t}(d,x) \int_{0}^{\infty}  \mu^{o'}_{0}(d,x) \left( KL_{d,x}(\theta)   \leq v \right) e^{-N_{t}(d,x)v + t r_{t} } dv   }  
	\end{align*}
	where the second line(s) follow from a change of variable. Finally, it is easy to see that $u \mapsto \mu^{o}_{0}(d,x) \left(   KL_{d,x}(\theta)  \leq u   \right)  = : G_{d,x}(u)$ is a CDF.  
\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:alpha.bound} ]
	Note that $\phi( m_{t}(d,x) ; \zeta^{o}_{0}(d,x) , ( N_{t}(d,x)  + \nu^{o}_{0}(d,x)  )/( N_{t}(d,x)\nu^{o}_{0}(d,x) ) )  =  \phi( \bar{m}_{t}(d,x) - \bar{\zeta}^{o}_{0}(d,x) ; 0 , \sigma^{2}_{t}(d,x)) $, where $\sigma^{2}_{t}(d,x) : = ( N_{t}(d,x)  + \nu^{o}_{0}(d,x)  )/( N_{t}(d,x)\nu^{o}_{0}(d,x) ) $ and $\bar{.}$ indicates centered at $\theta(d,x)$.  
	
	Under $| \bar{m}_{t}(d,x) | \leq \delta$, if follows that 
	\begin{align*}
		(\bar{m}_{t}(d,x) - \bar{\zeta}^{o}_{0}(d,x) )^{2}  = &  ( \bar{m}_{t}(d,x)  )^{2} + (\bar{\zeta}^{o}_{0}(d,x) )^{2}  - 2 \bar{m}_{t}(d,x) \bar{\zeta}^{o}_{0}(d,x)   \\
		\leq & \delta^{2} + (\bar{\zeta}^{o}_{0}(d,x) )^{2}  - 2 \bar{m}_{t}(d,x)  \bar{\zeta}^{o}_{0}(d,x) \\
		\leq & \delta^{2} + (\bar{\zeta}^{o}_{0}(d,x) )^{2}  + 2 | \bar{m}_{t}(d,x) |  |\bar{\zeta}^{o}_{0}(d,x) |\\
		\leq &  \delta^{2} + (\bar{\zeta}^{o}_{0}(d,x) )^{2}  + 2 \delta  |\bar{\zeta}^{o}_{0}(d,x) | \\
		= & (  \delta + |\bar{\zeta}^{o}_{0}(d,x) |    )^{2}
	\end{align*}
	
	
	Therefore, 
	\begin{align*}
		\log  \phi( \bar{m}_{t}(d,x) - \bar{\zeta}^{o}_{0}(d,x) ; 0 , \sigma^{2}_{t}(d,x))  \geq &  - \log   \sigma_{t}(d,x)  - 0.5  \frac{ (  \delta + |\bar{\zeta}^{o}_{0}(d,x) |    )^{2}    }  {   \sigma^{2}_{t}(d,x) } + Cte\\
		= & 	\log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \sigma^{2}_{t}(d,x))  + Cte,
	\end{align*}
	where $Cte$ is an irrelevant constant. 
	
	
	
	
	
	
	Observe that $\sigma \mapsto \log  \phi( y ; 0 , \sigma^{2})   $ is such that $\frac{d \log  \phi( y ; 0 , \sigma^{2})   } {d\sigma} = - \sigma^{-1} + \sigma^{-3} y^{2}   = \sigma^{-1} \left(  \sigma^{-2} y^{2}  - 1    \right)     $, so it is decreasing if $y^{2} < \sigma^{2}$ and increasing if $y^{2} > \sigma^{2}$.  Also, under $|f_{t}(d,x) - \pi_{t}(d,x)| \leq \eta$, 
	\begin{align*}
		& \sigma^{2}_{t}(d,x)  \geq 	\underline{\sigma}^{2}_{t}(d,x) : = 1/\nu^{o}_{0}(d,x) + t^{-1}/(\pi_{t}(d,x) + \eta)  \\
		~and~	& \sigma^{2}_{t}(d,x)  \leq 	\overline{\sigma}^{2}_{t}(d,x) : = 1/\nu^{o}_{0}(d,x) + t^{-1} /(\pi_{t}(d,x) - \eta)  .
	\end{align*} 
	Hence, if $(\delta + |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} < \sigma^{2}_{t}(d,x)$  then 
	\begin{align*}
		\log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \sigma^{2}_{t}(d,x))    \geq	\log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \overline{\sigma}^{2}_{t}(d,x))   
	\end{align*}
	if $(\delta+ |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} > \sigma^{2}_{t}(d,x)$  then 
	\begin{align*}
		\log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \sigma^{2}_{t}(d,x))    \geq	\log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \underline{\sigma}^{2}_{t}(d,x))  . 
	\end{align*}
	Hence a possible lower bound is given by 
	\begin{align*}
		\underline{\ell}( \eta ,\delta,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) ,  \pi_{t}(d,x)  ) : =  & 1\{ (\delta + |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} < \overline{\sigma}^{2}_{t}(d,x) \}     \log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \overline{\sigma}^{2}_{t}(d,x))    \\
		& +    1\{ (\delta + |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} > \underline{\sigma}^{2}_{t}(d,x) \} 	\log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \underline{\sigma}^{2}_{t}(d,x))    \} .
	\end{align*}
	To verify this is a valid lower bound, note that $(\delta + |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} < \sigma^{2}_{t}(d,x)$ implies that $(\delta + |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} < \overline{\sigma}^{2}_{t}(d,x)$ and thus 
	\begin{align*}
		\underline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) ,  \pi_{t}(d,x)  ) =  \log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \overline{\sigma}^{2}_{t}(d,x)) 
	\end{align*}
	which by our previous displays is indeed a valid lower bound when $(\delta + |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} < \sigma^{2}_{t}(d,x)$. Similarly, if $(\delta + |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} \geq \sigma^{2}_{t}(d,x)$, then $(\delta + |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} \geq \underline{\sigma}^{2}_{t}(d,x)$ and 
	\begin{align*}
		\underline{\ell}( \delta , \eta,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) ,  \pi_{t}(d,x)  ) =  \log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \underline{\sigma}^{2}_{t}(d,x)) 
	\end{align*}
	which, again, by our previous calculations is a valid lower bound when $(\delta + |\bar{\zeta}^{o}_{0}(d,x) |   )^{2} > \sigma^{2}_{t}(d,x)$. 
	
	%
	%Hence,
	%\begin{align*}
	%	\log  \phi( \bar{m}_{t}(d,x) - \bar{\zeta}^{o}_{0}(d,x) ; 0 , \sigma^{2}_{t}(d,x))   \geq & \min\{  \log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \overline{\sigma}^{2}_{t}(d,x))    ,   	\log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \underline{\sigma}^{2}_{t}(d,x))    \} \\
	%	= : & \underline{\ell}( \delta , \eta,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) ,  \pi_{t}(d,x)  )
	%\end{align*}
	
	
	
	On the other hand, 
	\begin{align*}
		(\bar{m}_{t}(d,x) - \bar{\zeta}^{o}_{0}(d,x) )^{2}  \geq \max\{  (\bar{\zeta}^{o}_{0}(d,x) )^{2}  - 2 \delta |\bar{\zeta}^{o}_{0}(d,x) | , 0 \}. 
	\end{align*}
	Therefore, 
	\begin{align*}
		\log  \phi( \bar{m}_{t}(d,x) - \bar{\zeta}^{o}_{0}(d,x) ; 0 , \sigma^{2}_{t}(d,x))  \leq &  - \log   \sigma_{t}(d,x)  - 0.5  \frac{  \max\{  (\bar{\zeta}^{o}_{0}(d,x) )^{2}  - 2 \delta |\bar{\zeta}^{o}_{0}(d,x) | , 0 \}   }  {   \sigma^{2}_{t}(d,x) } + Cte\\
		\leq &  - \log   \underline{\sigma}_{t}(d,x)  - 0.5  \frac{  \max\{  (\bar{\zeta}^{o}_{0}(d,x) )^{2}  - 2 \delta |\bar{\zeta}^{o}_{0}(d,x) | , 0 \}   }  {  \overline{ \sigma} ^{2}_{t}(d,x) } + Cte \\
		= : & \overline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) , \pi_{t}(d,x)   ).
	\end{align*}
\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:ell.properties}]
	(1) The proof is omitted as these property readily follows from Lemma \ref{lem:alpha.bound}.
	
	(2) We first observe that $\underline{\sigma}^{2}_{t}$ is decreasing as a function of $\eta$ and $\overline{\sigma}^{2}_{t}$ is increasing as a function of $\eta$. 
	
	Second, observe that $\overline{\ell}$ is decreasing as a function of $\underline{\sigma}^{2}_{t}$ and increasing as a function of $\overline{\sigma}^{2}_{t}$. Thus, $\overline{\ell}$ is increasing as a function of $\eta$. 
	
	Third, suppose $(\delta + |\bar{\zeta}^{o}_{0}(d,x)|)^{2} < \overline{\sigma}^{2}_{t}(d,x)$, then \begin{align*}
		\underline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) ,  \pi_{t}(d,x)  ) =     \log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \overline{\sigma}^{2}_{t}(d,x)). 
	\end{align*}
	Since $x \mapsto \log \phi(\delta + |\bar{\zeta}^{o}_{0}(d,x)|;0,x)$ is decreasing when $(\delta + |\bar{\zeta}^{o}_{0}(d,x)|)^{2} < x$, it follows that the RHS of the display is decreasing as a function of $\eta$. Now suppose $(\delta + |\bar{\zeta}^{o}_{0}(d,x)|)^{2} > \underline{\sigma}^{2}_{t}(d,x)$, then 
	\begin{align*}
		\underline{\ell}( \eta ,\delta ,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) ,  \pi_{t}(d,x)  ) =     \log  \phi( \delta ;  -  |\bar{\zeta}^{o}_{0}(d,x) |  , \underline{\sigma}^{2}_{t}(d,x)) 
	\end{align*}
	and since $x \mapsto \log \phi(\delta + |\bar{\zeta}^{o}_{0}(d,x)|;0,x)$ is increasing when $(\delta + |\bar{\zeta}^{o}_{0}(d,x)|)^{2} > x$ and $\underline{\sigma}^{2}_{t}(d,x)$ is decreasing as a function of $\eta$, it follows that the RHS of the display is decreasing as a function of $\eta$. 
	
	Hence, we showed that $	\underline{\ell}( \eta ,\delta,  |\bar{\zeta}^{o}_{0}(d,x) | , \nu^{o}_{0}(d,x) ,  \pi_{t}(d,x)  ) $ is decreasing as a function of $\eta$. 
	
	(3) Follows by inspection of $	\underline{\ell}$ and $\overline{\ell}$. 
	
	(4) The proof is omitted as these property readily follows from Lemma \ref{lem:alpha.bound}.
	
	(5) We do the proof for $\overline{\alpha}^{o}( \eta ,\delta ,  |\bar{\zeta}_{0}(d,x) | , \nu_{0}(d,x) , e_{t}(d,x) )$ as the proof of $\overline{\alpha}^{o}( \eta ,\delta ,  |\bar{\zeta}_{0}(d,x) | , \nu_{0}(d,x) )$ is analogous. By property 2, $\exp \overline{\ell}$ is increasing and $\exp \underline{\ell}$ is decreasing. As both these quantities are positive and $\overline{\alpha}^{o}( \eta ,\delta ,  |\bar{\zeta}_{0}(d,x) | , \nu_{0}(d,x) , e_{t}(d,x) )$ is essentially the ratio of the first over the second one, it follows that $\overline{\alpha}^{o}( \eta ,\delta ,  |\bar{\zeta}_{0}(d,x) | , \nu_{0}(d,x) , e_{t}(d,x) )$ is increasing in $\eta$. A similar argument delivers increasing in $\delta$. 
\end{proof}


==> app_mixing.tex <==
\section{Stochastic Properties of the Bayesian Posteriors and weights}



\textbf{Timing.} We first recall the timing. At period $t \in \{1,..., T, ...\}$, the planner starts with beliefs $(\zeta^{o}_{t-1},\nu^{o}_{t-1})_{o=0}^{L}$ and weights $(\alpha^{o}_{t-1})_{o=0}^{L}$, it takes an action $D_{t}$, the corresponding outcome is realized $Y_{t}(D_{t})$ and beliefs are updated given this new information. 

\bigskip  


The next lemma shows that for any $t$ and any $o \in \{0,...,L\}$, $\zeta^{o}_{t}$ can be written as a function of $(\zeta^{0}_{t},\nu^{0}_{t})$ and their priors, and the same holds for $\nu^{o}_{t}$. This result implies that it suffices to study the evolution of $(\zeta^{0}_{t},\nu^{0}_{t})_{t}$ and not of all the models. 

\begin{lemma}\label{lem:characterization.models}
	For any $t \geq 0$, any $o \in \{0,...,L\}$ and any $d \in \{0,...,M\}$, 
	\begin{align*}
		\nu^{o}_{t+1}(d) =  & \nu^{0}_{t+1}(d) - \nu^{0}_{0}(d)  + \nu^{o}_{0}(d) \\
		\zeta^{o}_{t+1}(d) = &  \frac{   \zeta^{0}_{t+1}(d) (\nu^{0}_{t+1}(d)  )    }{ \nu^{0}_{t+1}(d)   + \nu^{o}_{0}(d) - \nu^{0}_{0}(d)   }   + \frac{   \nu^{o}_{0}(d)  \zeta^{o}_{0}(d) -     \nu^{0}_{0}(d)  \zeta^{0}_{0}(d)    }{ \nu^{0}_{t+1}(d)   + \nu^{o}_{0}(d) - \nu^{0}_{0}(d)     }   
	\end{align*} 	
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:characterization.models} ]
	Throughout, we omit the super script "0" from the quantities. 
	
	Observe that for any $t \geq 1$, 
	\begin{align*}
		\nu_{t}(d) = \sum_{s=1}^{t} 1\{ D_{s}  = d \} + \nu_{0}(d) = \nu^{o}_{t}(d) + \nu_{0}(d)  - \nu^{o}_{0}(d).
	\end{align*}
	and 
	\begin{align*}
		\zeta_{t+1}(d) = & \frac{ 1\{D_{t+1} = d\} Y_{t+1}(d) }{ \nu_{t}(d) + 1\{ D_{t+1} = d  \}   }  +  \frac{ \nu_{t}(d)  \zeta_{t}(d) }{ \nu_{t}(d) + 1\{ D_{t+1} = d  \}   }   \\
		= & \frac{ 1\{D_{t+1} = d\} Y_{t+1}(d) }{ \nu_{t}(d) + 1\{ D_{t+1} = d  \}   } +   \frac{ 1\{D_{t} = d\} Y_{t}(d)   }{ \nu_{t}(d) + 1\{ D_{t+1} = d  \}   }   \\
		& +  \frac{ \nu_{t-1}(d)  \zeta_{t-1}(d) }{ \nu_{t}(d) + 1\{ D_{t+1} = d  \}   } 
	\end{align*} 
	since $\nu_{t}(d) = \nu_{t-1}(d) + 1\{ D_{t} = d\}$, and iterating in this fashion, it follows that
	\begin{align*}
		\zeta_{t+1}(d) = & \sum_{s=1}^{t+1}  \frac{ 1\{D_{s} = d\} Y_{s}(d) }{ \nu_{t}(d) + 1\{ D_{t+1} = d  \}   } +  \frac{ \nu_{0}(d)  \zeta_{0}(d) }{ \nu_{t+1}(d) + 1\{ D_{t+1} = d  \}   }.
	\end{align*}  
	Hence, $\sum_{s=1}^{t+1}   1\{D_{s} = d\} Y_{s}(d) = \zeta_{t+1}(d) (\nu_{t}(d) + 1\{ D_{t+1} = d  \}  )  -   \nu_{0}(d)  \zeta_{0}(d)  $. Since the same equation holds for $\zeta^{o}_{t+1}(d)$, it follows that 
	\begin{align*}
		\zeta_{t+1}(d) (\nu_{t}(d) + 1\{ D_{t+1} = d  \}  )  -   \nu_{0}(d)  \zeta_{0}(d)  =  \zeta^{o}_{t+1}(d) (\nu^{o}_{t}(d) + 1\{ D_{t+1} = d  \}  )  -   \nu^{o}_{0}(d)  \zeta^{o}_{0}(d), 
	\end{align*}
	which implies \begin{align*}
		\zeta^{o}_{t+1}(d) = & \frac{   \zeta_{t+1}(d) (\nu_{t+1}(d)   )    }{ \nu^{o}_{t+1}(d)    }   + \frac{   \nu^{o}_{0}(d)  \zeta^{o}_{0}(d) -     \nu_{0}(d)  \zeta_{0}(d)    }{ \nu^{o}_{t+1}(d)    } \\
		= &  \frac{   \zeta_{t+1}(d) (\nu_{t+1}(d)   )    }{ \nu_{t+1}(d)   + \nu^{o}_{0}(d) - \nu_{0}(d)   }   + \frac{   \nu^{o}_{0}(d)  \zeta^{o}_{0}(d) -     \nu_{0}(d)  \zeta_{0}(d)    }{ \nu_{t+1}(d)  + \nu^{o}_{0}(d) - \nu_{0}(d)     }  
	\end{align*}
\end{proof}

The next lemma shows that $\alpha^{o}_{t}$ can also be written as a function of  $\zeta^{0}_{t}$ and $\nu^{0}_{t}$, and the priors. 

\begin{lemma}\label{lem:characterization.alpha} 
	For any $t \geq 0$, any $o \in \{0,...,L\}$ and any $d \in \{0,...,M\}$, 
	\begin{align*}
		\alpha^{o}_{t}(d) =  \frac{   \exp  \ell^{o}_{t}(d)   }   {    \sum_{o=0}^{L}  \exp  \ell^{o}_{t}(d)      }    
	\end{align*}
where 
\begin{align*}
	& \ell^{o}_{t}(d) \\
	  = & \log \phi  ( \frac{\nu^{0}_{t}(d)} { \nu^{0}_{t}(d) - \nu^{0}_{0}(d)  }   \zeta^{0}_{t}(d) -  \frac{\nu^{0}_{0}(d)} { \nu^{0}_{t}(d)  - \nu^{0}_{0}(d) }  \zeta^{0}_{0}(d)    ;  \zeta^{o}_{0}(d) ,   ( \nu^{0}_{t}(d) - \nu^{0}_{0}(d)  + \nu^{o}_{0}(d)  )/( ( \nu^{0}_{t}(d) - \nu^{0}_{0}(d)    ) \nu^{o}_{0}(d) )    ) .
\end{align*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:characterization.alpha} ]
	Throughout we omit the super script "0" from the relevant quantities. 
	
	
	It readily follows from the fact that $\zeta_{t}(d) =  \frac{N_{t}(d)} { \nu_{t}(d)  }  m_{t}(d) + \frac{\nu_{0}(d)} { \nu_{t}(d)  }  \zeta_{0}(d)    $ iff $ \frac{\nu_{t}(d)} { N_{t}(d)  }   \zeta_{t}(d) -  \frac{\nu_{0}(d)} { N_{t}(d)  }  \zeta_{0}(d)    = m_{t}(d)  $ and $N_{t}(d) = \nu_{t}(d) - \nu_{0}(d)$. 
\end{proof}


\subsection{The Markov Chain for $(Z_{t})_{t}$}
	Throughout we omit the super script "0" from $(\zeta^{0}_{t},\nu^{0}_{t})$.

For each $t$, let $$Z_{t} : = (\zeta_{t},\nu_{t}) \in \mathbb{Z};$$ we now define the state space, $\mathbb{Z}$. To do this, first let, for any $t \in \{0,...,T\}$,
\begin{align*}
	%	\mathcal{V}_{t}   : = & \{ a \in \{0,1,...,t \}^{M+1}  \colon \sum_{d=0}^{M} a(d) < t  \},\\
	% \partial \mathcal{V}_{t}   : = & \{ a \in \{0,1,...,t \}^{M+1}  \colon \sum_{d=0}^{M} a(d) = t  \},\\
	%  \bar{\mathcal{V}}_{t}  : =  &	\mathcal{V}_{t}   \cup \partial 	\mathcal{V}_{t}   =  \{ a \in n \{0,1,...,t \}^{M+1}    \colon \sum_{d} a(d)  \leq t  \} \\
	%  ~and~ 
	\mathcal{V}_{t}(\nu_{0}) : =  	&   \{ a \in \{ \nu_{0} ,1 + \nu_{0} ,...,t+ \nu_{0}  \}^{M+1}  \colon \sum_{d=0}^{M} a(d) -  \nu_{0} < t  \}  \\
	\partial  \mathcal{V}_{t}(\nu_{0}) : = &	\{ a \in \{ \nu_{0} ,1 + \nu_{0} ,...,t+ \nu_{0}  \}^{M+1}  \colon \sum_{d=0}^{M} a(d) -  \nu_{0}  = t  \}  \\
	\bar{\mathcal{V}}_{t}(\nu_{0}) : = &  \mathcal{V}_{t} (\nu_{0})  \cup \partial 	\mathcal{V}_{t} (\nu_{0}). 
\end{align*}
Note that $\nu_{t} \in \bar{\mathcal{V}}_{T}(\nu_{0}) $ and if $\nu_{t} \in  \partial \mathcal{V}_{T}(\nu_{0}) $, then $\sum_{d} 1\{D_{t} = d \} = T$ and thus the experiment stops.  Hence, $\mathbb{Z} : = \mathbb{R}^{M+1} \times  \bar{\mathcal{V}}_{T}(\nu_{0}) $. Henceforth, we will omit $\nu_{0}$ from the set $\mathcal{V}_{T}$. 

Henceforth, we will omit $\nu_{0}$ from the set $\mathcal{V}_{T}$.


The policy functions $\phi : = (\sigma,\delta)$ --- that are time homogeneous --- and the DGP for $Y$ induce a Markov chain over $(Z_{t})_{t}$ with transition probability function $Q$. This transition probability function is characterize by the following recursion: For any $d \in \{0,...,M\}$ and given $z_{t} = (\zeta_{t},\nu_{t} )$, 
\begin{align*}
	\nu_{t+1}(d) = & 	\nu_{t}(d)  + 1\{ D_{t+1} = d   \} 1\{  \nu_{t} \in \mathcal{V}_{T}(\nu_{0})   \} \\
	\zeta_{t+1}(d) = & \frac{ 1\{D_{t+1} = d\} Y_{t+1}(d) }{ \nu_{t}(d) + 1\{ D_{t+1} = d  \}   }  +  \frac{ \nu_{t}(d)  \zeta_{t}(d) }{ \nu_{t}(d) + 1\{ D_{t+1} = d  \}   }, 
\end{align*}
where $\Pr( D_{t+1} = d \mid z_{t}) = \delta(z_{t}) (d)$ and $Y_{t+1}(d) \sim F_{d}$ where $F_{d}$ has mean $\theta(d)$, variance $\sigma^{2}(d)$ and, by Assumption \ref{ass:sub-gauss}, it is assumed to have full support PDF and to be sub-gaussian, i.e., $E[\exp \lambda ( Y(d)  - \theta(d))  ] \leq C \exp \upsilon \sigma^{2}(d)  \lambda^{2} $ for some constants $C=1$, $\upsilon > 0$  and any $\lambda>0$.


\subsection{Properties of the transition probability function $Q$}
\label{app:properties.Q} 


We now prove certain useful properties of $Q$.  For this, let $\mathbf{1}_{z}(.)$ be the Dirac probability measure at $z$.  Also, we now define a family of conditional probability measures over $\mathbb{Z}$. For any $m \in \{0,...\}$ and $z_{0} =(\zeta_{0},\nu_{0}) \in \mathbb{Z}$, let $\mathcal{Q}_{m}(.|z_{0})$ be such that 
\begin{align*}
	\mathcal{Q}_{m}( A_{\zeta} \times A_{\nu}  \mid  z_{0} ) :  = \mathbf{1}_{ \{ \nu_{0}(m) +  1\{  \nu_{0}(.) \in \mathcal{V}_{T-m} \} \}  }  ( A_{\nu}    )   Q( \zeta(m) \in A_{\zeta}   \mid  D = m, z_{0}(m)  ),
\end{align*}
for all $A_{\zeta} \times A_{\nu}$ Borel in $\mathbb{Z}$. 

\subsubsection{Small sets}

In this section we characterize the type of sets that are ``small", i.e., a set $C$ such that there exists a $\delta>0$, a $n \in \mathbb{N}$, and a measure $\psi \in \Delta(\mathbb{Z})$ such that 
\begin{align*}
	\inf_{z \in C }   Q^{n}(\cdot \mid z) \geq \delta \psi(.).
\end{align*}

The next lemma provides a simple lower bound for $Q$ using the fact that $\delta(.)(.) \geq \epsilon$.

\begin{lemma}\label{lem:Q.lower.bound.0}
	For any set $A : = \prod_{m=1}^{M} A(m)$ and any $z_{0} \in \mathbb{Z}$, it follows that 
			\begin{align*}
		Q^{L+1} (A \mid z_{0}) \geq \epsilon   \int  Q^{L}(A \mid z_{1})  Q(dz_{1} \mid D_{0} = d_{0}, z_{0}),~\forall L\geq 0~and~d_{0} \in \{0,...,M\},
	\end{align*} 
	and 
	\begin{align*}
		Q(A \mid z_{0})  \geq  \epsilon \sum_{l=0}^{M}   \prod_{d \ne l} \mathbf{1}_{ z_{0} (d)  }( A(d)   ) Q( A(l)  \mid  D = l, z_{0} ).
	\end{align*}   
\end{lemma}	

\begin{proof}[Proof of Lemma \ref{lem:Q.lower.bound.0}] 
	First we observe that for any $L \in \{0,..., M\}$, any $z_{0}$ and any set $A$, 
	\begin{align*}
		Q^{L+1} (A \mid z_{0}) =  &   \int Q^{L}(A \mid z_{1})  Q(dz_{1} \mid z_{0})  \\
		= &  \int \sum_{d_{0} }   \delta(z_{0})(d_{0})     Q^{L}(A \mid z_{1})  Q(dz_{1} \mid D_{0} = d_{0}, z_{0}) \\
		\geq & \epsilon  \int      Q^{L}(A \mid z_{1})  \sum_{d_{0}} Q(dz_{1} \mid D_{0} = d_{0}, z_{0}), 
	\end{align*} 
	where $Q^{0}(.\mid z) : = \mathbf{1}_{z}(.)$ and the third line follows because $\delta(.)(.) \geq \epsilon$. Observe further that for any $d \in \{0,...,M\}$, 
	\begin{align*}
		Q( A  \mid D_{0} = d, z_{0})  = \prod_{d' \ne d} \mathbf{1}_{z_{0}(d')}(A(d')) Q( A(d)  \mid  D_{0} = d, z_{0} ).
	\end{align*}
	Thus, for $L=0$, this implies that 
	\begin{align*}
		Q (A \mid z_{0}) 	\geq  \epsilon \sum_{d=0}^{M}  \prod_{d' \ne d} \mathbf{1}_{z_{0}(d')}(A(d')) Q( A(d)  \mid  D_{0} = d, z_{0} ),
	\end{align*} 
\end{proof}



The next lemma show that we can lower bound the transition $Q^{L}$ for different values of $L \in \{0,...\}$ in terms of a product measure given by the family $(	\mathcal{Q}_{m})_{m}$.

\begin{lemma}\label{lem:Q.lower.bound}
	For any set $A : = \prod_{m=1}^{M} A(m)$ such that $A(m) : = A_{\zeta}(m) \times A_{\nu}(m)$, it follows that 
	\begin{enumerate}
		
		\item For any $z_{0} \in \mathbb{Z}$ and any $L \in \{1,...,M\}$,\footnote{$D_{t}$ is the random variable corresponding to the treatment assignment in period $t$; $z_{t}$ is the state at time $t$.}
		\begin{align*}
			Q^{L+1} (A \mid z_{0}) 	\geq  \epsilon^{L}  \int   Q(A \mid z_{1}(0),z_{2}(1),z_{3}(2),...,z_{L}(L-1),z_{0}(L),...,z_{0}(M))   \prod_{t=0}^{L-1}  \mathcal{Q}_{t}( dz_{t+1}(t)  \mid  z_{0} ). 
		\end{align*}	
		\item For any $z_{0} \in \mathbb{Z}$,
		\begin{align*}
			Q^{M+1} (A \mid z_{0}) 	\geq  \epsilon^{M+1}      \prod_{m=0}^{M}  \mathcal{Q}_{m}( A(m)   \mid  z_{0} ) ,
		\end{align*}
	\end{enumerate}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:Q.lower.bound}]
	
	
	
	(1)	By the proof of Lemma \ref{lem:Q.lower.bound.0}, for $ L \geq 1$ it follows that 
	\begin{align}\label{eqn:Petite-1}
		Q^{L+1} (A \mid z) 	\geq  \epsilon  \int    Q^{L}(A \mid z_{1}(0),z_{0}(1),...,z_{0}(M))  Q( dz_{1}(0)  \mid  D_{0} = 0, z_{0} ). 
	\end{align}
	
	Analogously, for any $z_{1}$,
	\begin{align*}
		Q^{L} (A \mid z_{1}) \geq & \epsilon  \int      Q^{L-1}(A \mid z_{2})  Q(dz_{2} \mid D_{1} = 1, z_{1}) \\
		\geq &  \epsilon  \int    Q^{L-1}(A \mid z_{1}(0),z_{2}(1),z_{1}(2),...,z_{1}(M))  Q( dz_{2}(1)  \mid  D_{1} = 1, z_{1}  ).  
	\end{align*}	
	Plugging this expression in \ref{eqn:Petite-1}  with $z_{1} = z_{1}(0),z_{0}(1),...,z_{0}(M)$,  it follows that 
	\begin{align*}
		Q^{L+1} (A \mid z_{0}) 	\geq &  \epsilon^{2}  \int   Q^{L-1}(A \mid z_{1}(0),z_{2}(1),z_{0}(2),...,z_{0}(M))  Q( dz_{2}(1)  \mid  D_{1} = 1,  z_{1}(0),z_{0}(1),...,z_{0}(M) )  \\
		&  \times Q( dz_{1}(0)  \mid  D_{0} = 0, z_{0} ). 
	\end{align*}	
	Since 
	\begin{align}\label{eqn:Petite-0} 
		Q( A(d)  \mid  D_{0} = d, z_{0} ) = \mathbf{1}_{ \{ \nu_{0}(d) + 1\{  \nu_{0}(.) \in \mathcal{V}  \}  \}   }(A_{\nu}(d)) Q(A_{\zeta}(d) \mid D_{0} = d, z_{0}(d)  ) ,
	\end{align}
	it follows that 
	\begin{align*}
		Q^{L+1} (A \mid z_{0}) 	\geq &  \epsilon^{2}  \int   Q^{L-1}(A \mid z_{1}(0),z_{2}(1),z_{0}(2),...,z_{0}(M))   \mathbf{1}_{ \{ \nu_{0}(1) + 1\{  \nu_{1}(.) \in \mathcal{V}_{T}   \}  \}   }( d\nu_{2}(1)   ) Q( d\zeta_{2}(1) \mid D_{1} = 1, z_{0}(1)  ) \\
		& \times   Q( dz_{1}(0)  \mid  D_{0} = 0, z_{0} ),
	\end{align*}	
	where $\nu_{1}(.) = ( \nu_{1}(0) , \nu_{0}(1),..., \nu_{0}(M)  ) = ( \nu_{0}(0) + 1\{ \nu_{0}(.) \in \mathcal{V}_{T}    \}, \nu_{0}(1),..., \nu_{0}(M)  ) $ because at time $0$, $D_{0} = 0$. Hence, $\nu_{1}(.) \in \mathcal{V}_{T}$ iff $\nu_{0} \in \mathcal{V}_{T-1}$. Thus, 
	\begin{align*}
		& Q^{L+1} (A \mid z_{0}) 	\\
		\geq &  \epsilon^{2}  \int   Q^{L-1}(A \mid z_{1}(0),z_{2}(1),z_{0}(2),...,z_{0}(M))   \mathbf{1}_{ \{ \nu_{0}(1) + 1\{  \nu_{0}(.) \in \mathcal{V}_{T-1}  \}  \}   }( d\nu_{2}(1)   )  \mathbf{1}_{ \{ \nu_{0}(0) + 1\{  \nu_{0}(.) \in \mathcal{V}_{T}  \}  \}   }( d\nu_{1}(0)   )  \\
		& \times Q( d\zeta_{1}(0) \mid D_{0} = 0, z_{0}(0)  )  Q( d\zeta_{2}(1) \mid D_{1} = 1, z_{0}(1)  )  \\
		= & \int   Q^{L-1}(A \mid z_{1}(0),z_{2}(1),z_{0}(2),...,z_{0}(M))  \mathcal{Q}_{1}( dz_{2}(1)   \mid z_{0}  )  \mathcal{Q}_{1}( dz_{1}(0)    \mid z_{0}  ) 
	\end{align*}	 
	
	Iterating in this fashion, it follows that
	\begin{align*}
		Q^{L+1} (A \mid z_{0}) 	\geq &  \epsilon^{L}  \int   Q(A \mid z_{1}(0),z_{2}(1),z_{3}(2),...,z_{L}(L-1),z_{0}(L),...,z_{0}(M))   \\
		& \times \prod_{t=0}^{L-1} \mathbf{1}_{ \{ \nu_{0}(t) +  1\{  \nu_{0}(.) \in \mathcal{V}_{T-t} \} \}  }  ( d\nu_{t+1}(t)   )  \prod_{t=0}^{L-1}  Q( d\zeta_{t+1}(t)  \mid  D_{t} = t, z_{0}(t)  ). 
	\end{align*}		
	
	
	(3)   In particular, for $L=M$, these results imply that 
	\begin{align*}
		Q^{M+1} (A \mid z_{0}) 	\geq &  \epsilon^{M}  \int   Q(A \mid z_{1}(0),z_{2}(1),z_{3}(2),...,z_{L}(M-1),z_{0}(M))   \\
		& \times \prod_{t=0}^{M-1} \mathbf{1}_{ \{ \nu_{0}(t) +  1\{  \nu_{0}(.) \in \mathcal{V}_{T-t} \} \}  }  ( d\nu_{t+1}(t)   )  \prod_{t=0}^{M-1}  Q( d\zeta_{t+1}(t)  \mid  D_{t} = t, z_{0}(t)  ) \\
		\geq &  \epsilon^{M+1}      \int  \prod_{t=0}^{M-1}  \mathbf{1}_{z_{t+1}(t)}(A(t)) Q( A(M)  \mid  D_{M} = M,  z_{1}(0),z_{2}(1),z_{3}(2),...,z_{L}(M-1),z_{0}(M))   \\
		& \times \prod_{t=0}^{M-1} \mathbf{1}_{ \{ \nu_{0}(t) +  1\{  \nu_{0}(.) \in \mathcal{V}_{T-t} \} \}  }  ( d\nu_{t+1}(t)   )  \prod_{t=0}^{M-1}  Q( d\zeta_{t+1}(t)  \mid  D_{t} = t, z_{0}(t)  ) \\
		\geq &  \epsilon^{M+1}      \int  \prod_{t=0}^{M-1}  \mathbf{1}_{z_{t+1}(t)}(A(t))  1_{ \{ \nu_{0}(M) +  1\{  \nu_{0}(.) \in \mathcal{V}_{T-M} \} \}  }  ( A_{\nu}(M)    )  Q( A_{\zeta}(M)  \mid  D_{M} = M, z_{0}(M)  )    \\
		& \times  \prod_{t=0}^{M-1} \mathbf{1}_{ \{ \nu_{0}(t) +  1\{  \nu_{0}(.) \in \mathcal{V}_{T-t} \} \}  }  ( d\nu_{t+1}(t)   )  \prod_{t=0}^{M-1}  Q( d\zeta_{t+1}(t)  \mid  D_{t} = t, z_{0}(t)  ) .
	\end{align*}	 
	And using our definitions, this implies that
	\begin{align*}
		Q^{M+1} (A \mid z_{0}) 	\geq & \epsilon^{M+1}   \int  \prod_{t=0}^{M}  \mathbf{1}_{z(t)}(A(t))   \mathcal{Q}( dz(0), ...,   dz(M-1)  , dz(M)  \mid  z_{0} ) \\
		= & \epsilon^{M+1}  \prod_{t=0}^{M}    	\mathcal{Q}_{t}( A(t) \mid z_{0} )  .
	\end{align*}
\end{proof}

The next lemma provides a lower bound for the probability  $	Q ( \cdot   \mid D = d, z_{0}  ) $ over $\mathbb{R}$, which in turn helps to construct a lower bound for $\mathcal{Q}_{m}$

\begin{lemma}\label{lem:Q.lower.bound.1} 
	For any $d \in \{0,...,M\}$ and any $C : = \prod_{m=0}^{M} C(m) \subseteq \mathbb{Z}$ where $C(d) : = C_{\zeta}(d) \times C_{\nu}(d)$, with $C_{\zeta}(d)$  bounded with non-empty interior, it follows that for any set $E \subseteq \mathbb{R}$
	\begin{align*}
		Q (  \zeta_{1}(d) \in E    \mid D = d, z  ) 	\geq  \delta_{C} Leb(E \mid C_{\zeta}(d) )  ,~\forall z  \in C
	\end{align*}
	where $$\delta_{C} : =  \inf_{y  \in C_{\zeta}(d)  } f_{d}(y) (1+\nu_{0}(d))$$
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:Q.lower.bound.1}]  
	
	Given $z$ and $D=d$, let $y \mapsto e(y,z(d)) : = \frac{ y }{1+ \nu(d) }   + \frac{\nu(d) }{1 + \nu(d) } \zeta(d)  $; also, recall that $y(d) \sim F_{d}$ with PDF $f_{d}$. Thus 
	\begin{align*}
		Q(\zeta_{1}(d) \in E   \mid D=d, z )  = & \int 1\{  e(y,z)  \in E  \}  F_{d}(dy) \\
		\geq &  \int 1\{  e(y,z)  \in E \cap C_{\zeta}(d)  \}   F_{d}(dy) \\
		\geq & \inf_{y \in C_{\zeta}(d)  } f_{d}(y) \int  1\{  e(y,z)  \in E \cap C_{\zeta}(d)  \} dy.
	\end{align*} 
	Observe that $de(y,z) = dy/(1+\nu(d))$. Thus, with a change of variables, 
	\begin{align*}
		Q(\zeta_{1}(d) \in E   \mid D=d, z )  	\geq &  (1+\nu(d))  \inf_{y  \in C_{\zeta}(d)  } f_{d}(y) \int  1\{  \zeta'(d)  \in E \cap C_{\zeta}(d)  \}  d\zeta'(d) \\
		\geq &  (1+\nu(d))  \inf_{y  \in C_{\zeta}(d)  } f_{d}(y) Leb( E \mid C_{\zeta}(d) )
	\end{align*}     
	where the last line follows from the fact that $Leb(C_{\zeta}(d)) \in (0,1]$. The result thus follows from the fact that $\nu(d) \geq \nu_{0}(d)$. 
	
	
	
	
	%XXXXXXXXXXXXXXXXXX
	%
	%%	Given $z$ and $D=d$, let $y \mapsto e(y,z(d)) : = \frac{ y }{1+ \nu(d) }   + \frac{\nu(d) }{1 + \nu(d) } \zeta(d)  $ and $y \mapsto g(y,z(d)) : =  \pi + \ell(y;z(d))$; also, recall that $y(d) \sim F_{d}$ with PDF $f_{d}$. Since $\zeta'(d) = e(Y(d),z(d))$, it follows that $\zeta'(d)$ has a PDF given by $g_{d}(.; z(d)) : = (1+\nu(d))f_{d}( (1+\nu(d)) \cdot - \zeta(d) )$. Importantly, $g_{d}(.; z(d))$ has full support. 
	%%	
	%%	
	%%	
	%%	
	%%	
	%%	Thus 
	%%		\begin{align*}
	%%		Q(\zeta_{1}(d) \in E ,~ \alpha_{1}(d) \in G  \mid D=d, z )  = & \int 1\{  e(y,z)  \in E  \} 1\{ g(y,z)  \in G  \}  F_{d}(dy) \\
	%%		\geq &  \int 1\{  e(y,z)  \in E \cap C_{\zeta}(d)  \} 1\{ g(y,z)  \in G \cap C_{\alpha}(d)  \}  F_{d}(dy) \\
	%%		\geq & \inf_{y \in C_{\zeta}(d) \cup C_{\alpha}(d) } f_{d}(y) \int  1\{  e(y,z)  \in E \cap C_{\zeta}(d)  \} 1\{ g(y,z)  \in G \cap C_{\alpha}(d)  \}  dy.
	%%	\end{align*} 
	%%   
	%%   
	%%    Observe that $de(y,z) = dy/(1+\nu(d))$. Thus, with a change of variables, 
	%%		\begin{align*}
	%%	Q(\zeta_{1}(d) \in E ,~ \alpha_{1}(d) \in G  \mid D=d, z )  = & \int 1\{  e(y,z)  \in E  \} 1\{ g(y,z)  \in G  \}  F_{d}(dy) \\
	%%	\geq &  \int 1\{  e(y,z)  \in E \cap C_{\zeta}(d)  \} 1\{ g(y,z)  \in G \cap C_{\alpha}(d)  \}  F_{d}(dy) \\
	%%	\geq &  (1+\nu(d))  \inf_{\zeta'(d)  \in C_{\zeta}(d) \cup C_{\alpha}(d) } f_{d}(y) \int  1\{  \zeta'(d)  \in E \cap C_{\zeta}(d)  \} 1\{ g(y,z)  \in G \cap C_{\alpha}(d)  \}  d\zeta'(d).
	%%\end{align*}     
	%%	
	%%	
	%%	XXXXXXX
	%	
	%	
	%	
	%	Observe that, given $z=(\zeta,\nu)$ and $D=d$, $ \zeta_{1}(d) = \frac{ Y(d)  }{1+ \nu(d) }   + \frac{\nu(d) }{1 + \nu(d) } \zeta(d)  $, thus $ \zeta_{1}(d) $ is (conditionally) Gaussian with mean $ \frac{ \theta(d)  }{1+ \nu(d) }   + \frac{\nu(d) }{1 + \nu(d) } \zeta(d)  $ and variance $1/(1+\nu(d))^{2}$. Thus,
	%	\begin{align*}
	%		Q(\zeta_{1}(d) \in S \mid D=d, z )  = & \int_{S}     \phi( w ; \frac{ \theta(d)  }{1+ \nu(d) }   + \frac{\nu(d) }{1 + \nu(d) } \zeta(d)  ,  1/(1+\nu(d))^{2}  ) dw \\
	%		= & \int_{S( \zeta(d) , \nu(d)  ) }      \phi ( (1+\nu(d)) w  - \zeta(d) \nu(d) , \theta(d),\sigma^{2}(d)  )  dw \\ 
	%		\geq & \int_{S( \zeta(d) , \nu(d)  )   \cap C(d)}     \phi ( (1+\nu(d)) w  - \zeta(d) \nu(d) , \theta(d),\sigma^{2}(d)  ) dw\\
	%		\geq &  \inf_{( \zeta_{1}(d) , \zeta(d), \nu(d) )  \in C(d) \times C}    \phi ( (1+\nu(d)) w  - \zeta(d) \nu(d) , \theta(d),\sigma^{2}(d)  )   Leb(S \cap C(d)),
	%	\end{align*}
	%	where $S( \zeta(d) , \nu(d)  ) $ is the inverse image of the mapping $y \mapsto \frac{ y  }{1+ \nu(d) }   + \frac{\nu(d) }{1 + \nu(d) } \zeta(d)  $, and it still bounded.  Since $C$ is bounded and $\phi$ has full support, it follows that $\inf_{( \zeta_{1}(d) , \zeta(d), \nu(d) )  \in C(d) \times C(d)}   \phi ( (1+\nu(d)) w  - \zeta(d) \nu(d) , \theta(d),\sigma^{2}(d)  )   = : \delta_{C} > 0$. The result follows as $0 < Leb(C(d)) \leq 1$.
\end{proof}

\begin{lemma}\label{lem:small}
	Any set $\mathcal{C} = \prod_{m=0}^{M} \mathcal{C}(m)$ where $\mathcal{C}(m) : =  \{ (\zeta(m),\nu(m)) \colon  \zeta(m) \in  S(m),~ \nu(m) = a  \} $ with $S(m)$ bounded and with non-empty interior and $a(.) \in \bar{\mathcal{V}}_{T}(\nu_{0})$ is small, i.e., 
	\begin{align*}
		Q^{M+1}(A \mid z) \geq \epsilon^{M+1} \delta_{\mathcal{C}}  \psi(A),~\forall A \subseteq \mathbb{Z},
	\end{align*}
	for any $z \in \mathcal{C}$, where $\psi$ is a probability measure such that
	\begin{align*}
		\psi(A) & =  \prod_{m=0}^{M}    \mathbf{1}_{a(m)+1\{ m < m^{\ast}  \}} (A_{\nu} (m)   )  Leb(A_{\zeta}(m)  \mid  \mathcal{C}(m) ),
	\end{align*}
	for any set $A : = \prod_{m=0}^{M} A_{\zeta}(m) \times A_{\nu}(m)$, where $m^{\ast}$ be the first $m \in \{0,...,M\}$ such that $a(.) \notin \mathcal{V}_{T-m}$ (if this never happens, we simply set $m^{\ast} = T$).
\end{lemma}


\begin{proof}[Proof of Lemma \ref{lem:small}]
	Abusing notation, let $Q(\cdot \mid D=d , z)$ be the probability over $\mathbb{Z}$ given $D=d$ and $Z=z$.
	
	Let $m^{\ast}$ be the first $m \in \{0,...,M\}$ such that $a(.) \notin \mathcal{V}_{T-m}$ (if this never happens, we simply set $m^{\ast} = T$).
	
	It is enough to show the results for ``squares", $A : = \prod_{m=0}^{M} A(m)$ and $A(m) : =  A_{\zeta}(m)  \times A_{\nu}(m)  $ with $A_{\nu}(m) \subseteq \{ 1,...,T \}$ and $A_{\zeta}(m) \subseteq \mathbb{R}$. 
	
	First assume $a(.) \in \mathcal{V}_{T}$, then by Lemma \ref{lem:Q.lower.bound}(2) 
	\begin{align*}
		Q^{M+1} (A \mid z_{0}) 	\geq &  \epsilon^{M+1}      \prod_{m=0}^{M}  \mathcal{Q}_{m}( A(m)   \mid  z_{0}) \\
		= &   \epsilon^{M+1}      \prod_{m=0}^{m^{\ast}-1}  \mathcal{Q}_{m}( A(m)   \mid  z_{0})  \prod_{m=m^{\ast}}^{M}  \mathcal{Q}_{m}( A(m)   \mid  z_{0}) 
	\end{align*} 
	(if $m^{\ast} = 0$, then the first product is taken to be 1 and if $m^{\ast} > M$ the second product is taken to be 1). 
	
	Recall that for $z_{0}$ in $\mathcal{C}$, $\nu_{0}(.) = a(.)$. Hence, for each $m \in \{0,...,m^{\ast}-1\}$,
	\begin{align*}
		\mathcal{Q}_{m}( A(m)   \mid  z_{0}) = 	\mathbf{1}_{ a(m) +  1   }  ( A_{\nu}(m)    )   Q( \zeta(m) \in A_{\zeta} (m)  \mid  D = m, z_{0}(m)  )
	\end{align*}
	and for each $m \in \{m^{\ast},...,M \}$,
	\begin{align*}
		\mathcal{Q}_{m}( A(m)   \mid  z_{0}) = 	\mathbf{1}_{ a(m) }  ( A_{\nu} (m)   )   Q( \zeta(m) \in A_{\zeta} (m)  \mid  D = m, z_{0}(m)  ).
	\end{align*}
	
	By Lemma \ref{lem:Q.lower.bound.1}, it follows that, for each $m \in \{0,...,m^{\ast}-1\}$,  
	\begin{align*}
		Q( \zeta(m) \in A_{\zeta}(m)   \mid  D = m, z_{0}(m)) \geq  \mathbf{1}_{a(m)+1} ( A_{\nu}(m)   ) \delta_{\mathcal{C}(m)} Leb( A_{\zeta} (m ) \mid \mathcal{C}(m)   ),
	\end{align*}
	and for each $m \in \{m^{\ast},...,M \}$,
	\begin{align*}
		\mathcal{Q}_{m}( A(m)   \mid  z_{0}) \geq  	\mathbf{1}_{ a(m) }  ( A_{\nu} (m)   )  \delta_{\mathcal{C}(m)} Leb( A_{\zeta} (m ) \mid \mathcal{C}(m)   ).
	\end{align*}
	Hence, 
	\begin{align*}
		Q^{M+1} (A \mid z_{0}) 	\geq  \epsilon^{M}      \prod_{m=0}^{M} \delta_{\mathcal{C}(m)}  \mathbf{1}_{a(m)+1\{ m < m^{\ast} \}} ( A_{\nu}(m)   ) Leb( A_{\zeta} (m ) \mid \mathcal{C}(m)   ) 
	\end{align*}  	
	letting $\delta_{\mathcal{C}}  : = \min_{m} \delta_{C(m)} > 0$, the result follows. 
\end{proof}

\begin{remark}[A remark about Assumption \ref{ass:PF.epsilon}]
	By inspection of the proof of Lemma \ref{lem:small}, and the other lemmas used as building blocks, it follows that Assumption \ref{ass:PF.epsilon} could be relaxed to allow for $\epsilon$ to depend on the state, i.e., $z \mapsto \epsilon(z)$ provided that $\inf_{z \in C} \epsilon(z) > 0$ for any $C$ compact. $\triangle$ 
\end{remark}



\subsubsection{Drift Condition }

In this section we show that $Q$ satisfies a drift condition. 

\begin{lemma}\label{lem:Q.drift}
	For any $a \geq 0$ and $A \geq 0$, the function $z \mapsto V(z) : = 1 + a ||\bar{\zeta}||_{1} + A  ||\nu - \partial \mathcal{V}_{T} ||_{1}$ where $d \mapsto \bar{\zeta}(d) : = (\zeta(d) - \theta(d))/\sigma(d) $, satisfies 
	\begin{align*}
		Q[V](z) \leq  \gamma(z) V(z) + b,
	\end{align*}
	with $\gamma(z) : = \epsilon \max_{d} \frac{\nu(d) }{\nu(d) +1} + (1-\epsilon) $ and $b : = 1-\gamma + a \sum_{d}  \frac{ \delta(z)(d)   }{1 + \nu_{0}(d) }   $.  Observe that $\max_{z} \gamma(z) \leq \gamma : = \epsilon \max_{d} \frac{\nu_{0}(d) +  T}{\nu_{0}(d) + T +1} + (1-\epsilon) < 1$. 
\end{lemma}

\begin{proof}
	Suppose $z$ is such that $||\nu||_{1} = T-l$ for some $l \in \{1,...,T\}$. 
	
	It follows that 
	\begin{align*}
		Q[V](z) = & 1 + a \int ||\bar{\zeta}' ||_{1} Q(d\zeta' \mid z )  + A \int ||\nu' - \partial \mathcal{V}_{T} ||_{1} Q(d\nu' \mid z ) \\
		= & 1 + a \sum_{d} \delta(z)(d)  \int \left( |\bar{\zeta}'(d)|   + \sum_{m \ne d}  |\bar{\zeta}(m)|  \right) Q(d\zeta' \mid D=d, z )  \\
		& + A \sum_{d} \delta(z)(d) \int ||(\nu'(d),\nu(-d)) - \partial \mathcal{V}_{T} ||_{1}  Q(d\nu' \mid D=d, z ). 
	\end{align*}
	where $(\nu'(d),\nu(-d)) $ denotes the vector where the $d$-th coordinate is $\nu'(d)$ and the rest of the coordinates are given by $\nu(-d)$. Because $||\nu||_{1} = T-l$, it follows that $||(\nu(d)+1,\nu(-d))||_{1} = T-l-1$ and thus $||(\nu(d)+1,\nu(-d)) - \mathcal{V}_{T} ||_{1} = l-1 \leq \frac{T-1}{T} ||\nu - \mathcal{V}_{T} ||_{1}  $.  Moreover, if $l=0$, then $\nu'(d) = \nu(d)$ and $||(\nu'(d),\nu(-d)) - \mathcal{V}_{T} ||_{1} = 0$. 
	
	Also, observe that $|\bar{\zeta}'(d)| \leq |\bar{y}|/(1 + \nu(d))  + |\bar{\zeta}(d)| \nu(d)/(1 + \nu(d))|$ and $\nu(d) \geq \nu_{0}$. Thus, 
	\begin{align*}
		& \sum_{d} \delta(z)(d)  \int \left( |\bar{\zeta}'(d)|   + \sum_{m \ne d}  |\bar{\zeta}(d)|  \right) Q(d\zeta' \mid D=d, z ) \\
		\leq &  |\bar{\zeta}(0)| \left( \sum_{d}  \delta(z)(d)  \omega(d,0)    \right) + ... +  |\bar{\zeta}(M)| \left( \sum_{d}  \delta(z)(d)  \omega(d,M)    \right) \\
		& + a \sum_{d}  \frac{ \delta(z)(d)   }{1 + \nu(d) }   \int |\bar{y}|  f_{d} ( y )  dy
	\end{align*}
	where $\omega(d',d) = 1$ if $d' \ne d$ and $=( \nu(d) )/(1+ \nu(d) )$ if $d'=d$. Hence, for any $m$, $ \sum_{d}  \delta(z)(d)  \omega(d,m) =  \delta(z)(m)  \frac{ \nu(m) }{1+ \nu(m) } + (1-\delta(z)(m))  \leq \epsilon   \frac{ \nu(m) }{1+ \nu(m) } + (1-\epsilon) : = \gamma(\nu(m)) $ because $\delta(z)(d) \geq \epsilon$ by Assumption \ref{ass:PF.epsilon}. Let $\gamma(\nu) : = \max_{m} \gamma(\nu(m))$.  Thus
	\begin{align*}
		Q[V](z) = & 1 + a \int ||\bar{\zeta}' ||_{1} Q(d\zeta' \mid z )  + A \int ||\nu' - \partial \mathcal{V}_{T} ||_{1} Q(d\nu' \mid z ) \\
		\leq & 1 + a \gamma(\nu) ||\bar{\zeta}||_{1} +  A \frac{T-1}{T} ||\nu - \partial \mathcal{V}_{T} ||_{1}  +  \sum_{d}  \frac{ \delta(z)(d)   }{1 + \nu(d) }   \int |\bar{y}|  \phi( y; \theta(d),1) dy\\
		\leq & \gamma(\nu) V(z) + (1-\gamma(\nu)) + a \sum_{d}  \frac{ \delta(z)(d)   }{1 + \nu(d) }   \int |\bar{y}|  f_{d} ( y ) dy.
	\end{align*}
	Since $ \int |\bar{y}|  f_{d} ( y ) dy \leq 1$ and $\nu(d) > \nu_{0}(d)$ the desired result follows. 	\end{proof}

\begin{lemma}
	Let $C \subseteq \mathbb{Z}$ and $a,A$ be as in Lemma \ref{lem:Q.drift} and let $\bar{\gamma}$ and $R : = \inf_{z \in C^{C}} V(z)$  be such that $\bar{\gamma} >  \gamma$ and 
	\begin{align*}
		\gamma   + 	(1 - \gamma + 0.5 a)/R  \leq   \bar{\gamma} 
	\end{align*}
	Then, for all $z \in \mathbb{Z}$, 
	\begin{align*}
		Q[V](z) \leq \bar{\gamma} V(z) + b 1_{C}(z) 
	\end{align*}	
\end{lemma}

\begin{proof}
	From Lemma \ref{lem:Q.drift}, for all $z \in \mathbb{Z}$,
	\begin{align*}
		Q[V](z) \leq \gamma V(z) + b,
	\end{align*}
	Thus
	\begin{align*}
		Q[V](z) \leq &\bar{\gamma} V(z)  - (   \bar{\gamma} - \gamma ) V(z)   +  b  \\
		\leq & \bar{\gamma} V(z)  - (   \bar{\gamma} - \gamma ) R   + b.
	\end{align*}
	
	We now show that $- (   \bar{\gamma} -  \gamma ) R   + b < 0$. To do this, note that 
	\begin{align*}
		- (   \bar{\gamma} -  \gamma ) R   + b = & (1-\gamma) + 0.5 a -  (   \bar{\gamma} -  \gamma ) R \\
		= &  1 +  \gamma (R-1) + 0.5 a -    \bar{\gamma} R.
	\end{align*}
\end{proof}


\begin{remark}\label{rem:Q.properties}
	Let
	\begin{align}
		\mathcal{C}  : = \prod_{m=0}^{M} \mathcal{C}(m) 
	\end{align}
	where $\mathcal{C}(m) : =  \{ (\zeta,\nu) \colon  |\bar{\zeta}(m)|   \leq (R/a)/(M+1)~and~\nu(m) = \mathbf{v}(m)   \}$ for some $\mathbf{v} \in \partial \mathcal{V}_{T}$ and $R > 0 $. By Lemma \ref{lem:small}, this set is small. 
	
	
	Moreover, $\inf_{z \in \mathcal{C}^{C}} V(z) \geq R+1$.  Note that since $\gamma < 1$, there exists  $R$ and $a$  	
	\begin{align*}
		\gamma   + b/(R+1)   = 	\gamma   + (	1 - \gamma + 0.5 a)/(R+1)  < 1 \iff \frac{0.5 a}{1-\gamma}   < R.
	\end{align*}
	$\triangle$ 
\end{remark}

%\begin{remark}[A remark about Assumption \ref{ass:PF.epsilon}]
%	If $\epsilon$ depends on the state $z$, then the statement of Lemma \ref{lem:Q.drift} will remain unchanged. The problem is that $\max_{z} \gamma(z)$ may not be less than $1$. To sidestep this issue, define $\tilde{V} : = \gamma V$ and note that \begin{align*}
%		Q[V](z) = E[V(z') | z] = E[ \gamma(z') V(z') / \gamma(z')  | z] = E[ \tilde{V} (z') / \gamma(z')  | z] 
%	\end{align*}
%	
%	
%	 $\triangle$ 
%\end{remark}



\subsubsection{Geometric Ergodicity} 
\label{app:ergodicity}



\begin{lemma}\label{lem:Q.GeoErgodic} 
	There exists a constant $L$ and an invariant distribution of $Q$, $\lambda$, such that, for any $n \geq 1$ and any $z_{0} \in \mathbb{Z}$,
	\begin{align*}
		||Q^{n}(.|z_{0})  - \lambda || \leq L V(z_{0}) e^{- n  \varrho(\epsilon)   } 
	\end{align*}
	where $\epsilon \mapsto \varrho(\epsilon)$ is positive valued, $\varrho(0) = 0$ and increasing on $\epsilon$; formally defined in the proof. 
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:Q.GeoErgodic}  ]
	This proof follows the proof of Theorems 9 and 12 in \cite{Roberts:2004} (RR).
	
	
	Lemma \ref{lem:small}  imply their condition 8 and Lemma \ref{lem:Q.drift}  with $\mathcal{C}$ chosen as in Remark \ref{rem:Q.properties} implies their condition 10.  Moreover, proposition 11 in RR holds with $\alpha: = \alpha(a,R,\gamma)^{-1} : =  \gamma   + (1-\gamma + 0.5 a )/(R+1)$, which by Remark \ref{rem:Q.properties}  is less than 1; moreover, it is increasing in $a$, decreasing in $R$ and decreasing on $\gamma$. Thus as pointed out in p. 47, their Theorem 12 holds. Thus,
	\begin{align*}
		||Q^{n}(.|z_{0})  - \pi || \leq & (1- \epsilon^{M+1} \delta_{\mathcal{C}}  )^{j}   + \alpha^{-n} B^{j-1}_{M} 0.5 ( V(z_{0}) + \int V(z) \pi(dz)   ) \\
		= :  & L V(z_{0})  \left(    (1- \epsilon^{M+1} \delta_{\mathcal{C}}  )^{j}   + \alpha^{-n} B^{j}_{M}     \right)
	\end{align*}
	for any $0 \leq j \leq n$, where $B_{M} : =   \max \{1  , \alpha^{M+1} (1- \epsilon^{M+1} \delta_{\mathcal{C}} )  \sup_{z \in \mathcal{C}} Q^{M+1}[V](z)      \}  $. 
	
	We now bound the term $ \alpha^{-n} B^{j}_{M} $. Observe that $\sup_{z \in \mathcal{C} } Q^{M+1}[V](z)   \leq \gamma^{M+1} \sup_{z \in \mathcal{C}} V(z) + \frac{1-\gamma^{M+1} }{1-\gamma} b   \leq \gamma^{M+1} ( (1+R) - b) + \frac{b}{1-\gamma}  $ (recall that $b = 1-\gamma  + 0.5 a$ and so \begin{align*}
		(1- \epsilon^{M+1} \delta_{\mathcal{C}} )  \sup_{z \in C} Q^{M+1}[V](z)   \leq 	(1- \epsilon^{M+1} \delta_{\mathcal{C}} )   \left( \gamma^{M+1} ( (1+R) - b) + \frac{b}{1-\gamma}    \right).
	\end{align*}
	Abusing notation, we redefine $\gamma$ as $\gamma: = \max\{ 	(1- \epsilon^{M+1} \delta_{\mathcal{C}} ) , \gamma  \}$ and let $R(a,\eta,\gamma) = 0.5a /(1-\gamma) + \eta$ for some $\eta>0$. It is easy to see that the previous display is bounded by 
	\begin{align*}	
		G( a, \eta , \gamma   ) : = & \gamma   \left( \gamma^{M+1} (  0.5a /(1-\gamma) + \eta  + \gamma - 0.5 a ) + 1 + 0.5a/(1-\gamma)   \right) \\
		= & \gamma   \left( \gamma^{M+1} (  0.5a \gamma /(1-\gamma) + \eta  + \gamma ) + 1 + 0.5a/(1-\gamma)   \right) , 
	\end{align*}
	which is increasing in all of its arguments.  Therefore,
	\begin{align*}
		\alpha^{-n} B^{j}_{M}  \leq \alpha(a,R(a,\eta,\gamma) ,\gamma)^{-n + j(M+1 + m)}  \left(  G( a, \eta, \gamma   ) /\alpha(a,R(a,\eta,\gamma),\gamma)^{m}   \right)^{j},~\forall m \in \mathbb{N}.
	\end{align*} 
	We note that 
	\begin{align*}
		G( 0, \eta, \gamma   ) =  \gamma   \left( \gamma^{M+1} ( \eta + \gamma  ) + 1   \right)  ~and~\alpha(0,R(0,\eta,\gamma) ,\gamma)^{-1} : =  \gamma   + (1-\gamma )/(\eta +1) <1.
	\end{align*}
	Therefore, there exists a $m : = m(\gamma,\eta)$ such that $G( 0, \eta, \gamma   ) /\alpha(0,R(0,\eta,\gamma),\gamma)^{m( \gamma ,\eta ) }  < 1$. It is straightforward to show that $m(.,.)$ is non-decreasing on $\gamma$ and non-decreasing on $\eta$ (at least for large values of $\eta$). By continuity, there exists a $a(\gamma,\eta)$ such that for all $a \leq a(\gamma,\eta)$, $G( a, \eta, \gamma   ) /\alpha(a,R(a,\eta,\gamma),\gamma)^{m(\gamma,\eta)}  \leq 1$. Moreover, $a(.,.)$ is non-increasing in $\gamma$. 
	
	Therefore, for any $\eta>0$ and $a \leq a(\gamma,\eta)$, it follows that 
	\begin{align*}
		\alpha^{-n} B^{j-1}_{M}  \leq \alpha(a,R(a,\eta,\gamma) ,\gamma)^{-n + j(M+1 + m( \gamma, \eta  )  )} .
	\end{align*} 
	By choosing $j = 0.5 n / (M+1 + m( \gamma, \eta  )  )  $ (if it is not an integer, simply take the floor), it follows that 
	\begin{align*}
		||Q^{n}(.|z_{0})  - \pi || \leq & L V(z_{0})) \alpha(a,R(a,\eta,\gamma) ,\gamma)^{   0.5 \frac{n}{  M+1 + m( \gamma, \eta  )   }     }   = L V(z_{0})) \exp \{  - 0.5 n  \frac{ \log \alpha^{-1}(a,R(a,\eta,\gamma) ,\gamma)   }{      M+1 + m( \gamma, \eta  )   }   \} 
	\end{align*}  
	Observe that by the computing the total derivative of $\gamma \mapsto \log \alpha^{-1}(a,R(a,\eta,\gamma) ,\gamma) $ with respect to $\gamma$ it can be shown that this function is decreasing on $\gamma$. Since $\gamma \mapsto m(\gamma,\eta)$ is non-decreasing, it follows that  $\gamma \mapsto  \frac{ \log \alpha^{-1}(a,R(a,\eta,\gamma) ,\gamma)   }{      M+1 + m( \gamma, \eta  )   } $  is decreasing on $\gamma$. Since $\gamma$ is decreasing on $\epsilon$ and increasing on $T$, it follows that $\epsilon \mapsto \varrho(\epsilon) : = \frac{ \log \alpha^{-1}(a,R(a,\eta,\gamma) ,\gamma)   }{      M+1 + m( \gamma, \eta  )   }$ is increasing on $\epsilon$.
\end{proof}	




\subsection{Mixing Results}\begin{lemma}\label{lem:mixing} 
	%	Let $\pi$ be any probability over $\mathbb{Z}$ such that $\int V(z) \pi(dz) < \infty$ (in particular, it could be different from $\lambda$). Then, there exists  a $\bar{\varrho} \in (0,1)$ such that the process $(Z_{t})_{t=1}^{\infty}$ with initial probabilty $\pi$ and transition $Q$ is $\beta$-mixing with mixing coefficients $k \mapsto \beta(k) = O( \bar{\varrho}^{k} )$.
	Let $\pi$ be any probability over $\mathbb{Z}$ such that $\int V(z) \pi(dz) < \infty$  (in particular, it could be different from  the invariant distribution $\lambda$). Then, the process $(Z_{t})_{t=1}^{\infty}$ with initial probabilty $\pi$  and transition $Q$ is $\beta$-mixing with mixing coefficients, $(\beta(k))_{k}$ such $\beta_{k} \leq C_{M} e^{ - k 0.5 \varrho(\epsilon)}$ for all $k \geq 1$, where 
	\begin{align*}
		C_{M} : = 3 \int V(z) \pi(dz) + \int V(z) \lambda(dz)
	\end{align*}
\end{lemma}
\label{app:mixing}


\begin{lemma}\label{lem:mixing} 
	%	Let $\pi$ be any probability over $\mathbb{Z}$ such that $\int V(z) \pi(dz) < \infty$ (in particular, it could be different from $\lambda$). Then, there exists  a $\bar{\varrho} \in (0,1)$ such that the process $(Z_{t})_{t=1}^{\infty}$ with initial probabilty $\pi$ and transition $Q$ is $\beta$-mixing with mixing coefficients $k \mapsto \beta(k) = O( \bar{\varrho}^{k} )$.
	Let $\pi$ be any probability over $\mathbb{Z}$ such that $\int V(z) \pi(dz) < \infty$  (in particular, it could be different from  the invariant distribution $\lambda$). Then, the process $(Z_{t})_{t=1}^{\infty}$ with initial probabilty $\pi$  and transition $Q$ is $\beta$-mixing with mixing coefficients, $(\beta(k))_{k}$ such $\beta_{k} \leq C_{M} e^{ - k 0.5 \varrho(\epsilon)}$ for all $k \geq 1$, where 
	\begin{align*}
		C_{M} : = 3 \int V(z) \pi(dz) + \int V(z) \lambda(dz)
	\end{align*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:mixing} ]
 See Propostion 4 in \cite{liebscher:2005}.
\end{proof}

\begin{proof}[Proof of Proposition \ref{pro:Z.mixing}]
	First, recall that $z = (\zeta^{0},\nu^{0})$ and Lemma \ref{lem:mixing} establishes that this process is $\beta$-mixing. Since, for all $o \in \{0,...,L\}$, $(\zeta^{o},\nu^{o},\alpha^{o})$ can be written as a deterministic function of $z$ (and the priors; see Lemmas \ref{lem:characterization.models} and \ref{lem:characterization.alpha}), conditional on the priors, the process $( \zeta_{t},\nu_{t},\alpha_{t} )_{t}$ is also $\beta$-mixing with the same convergence rate.
	
	By assumption, $\delta$ depends on $(\zeta^{o}_{t},\nu^{o}_{t},\alpha^{o}_{t})_{o=0}^{L}$ and thus it depends on $z_{t} = (\zeta^{0}_{t},\nu^{0}_{t})$ (and the priors, but these are taken to be non-random). Henceforth, and abusing notation, we use $z \mapsto \delta(z)$ to denote this composition of functions. 
		
	
	Note that for any $s \in \{0,1,...\}$, $1\{  D_{s} = d  \}  = 1\{  \delta(Z_{s})(d) \geq U_{s}  \} $ where $U_{s} \in U(0,1)$. It is easy to show that the ``expanded" process $(Z_{t},U_{t})_{t}$ is a Markov Chain with transition $Q \times U(0,1)$ and it inherits all the properties of the original one. In particular, by Lemma \ref{lem:mixing} , $(Z_{t},U_{t})_{t}$ is $\beta$-mixing with the same coefficients. Hence,  $(Z_{t},D_{t})_{t}$ is also a Markov Chain with transition $Q_{ext} $ and $\beta$-mixing with the same coefficients
	
	Since $Y_{t} = Y_{t}(D_{t})$ is a deterministic function of IID random variables, $(Y_{t}(d))_{d}$ and $D_{t}$. So to show that  $(Z_{t},D_{t},Y_{t})_{t}$ is $\beta$-mixing with the same coefficients, it suffices to show that $(Z_{t},D_{t},Y_{t}(0),...,Y_{t}(M) )_{t}$ is  $\beta$-mixing with the same coefficients.  It is easy to show that the ``expanded" process $(Z_{t},D_{t},Y_{t}(0),...,Y_{t}(M) )_{t}$  is a Markov Chain with transition $Q_{ext} \times F(0) \times ... \times F(M) $ and it inherits all the properties of the original one. In particular, by Lemma \ref{lem:mixing} , $(Z_{t},D_{t},Y_{t}(0),...,Y_{t}(M) )_{t}$ is $\beta$-mixing with the same coefficients. Therefore,   $(Z_{t},D_{t},Y_{t})_{t}$ is a Markov Chain and is $\beta$-mixing with mixing coefficients, $(\beta(k))_{k}$ such $\beta_{k} \leq C e^{ - 0.5 k \varrho(\epsilon)} $ for all $k \geq 1$. 
\end{proof}


==> tab_alpha.tex <==
% Table generated by Excel2LaTeX from sheet 'Main '
\begin{table}
  \centering
    \begin{threeparttable}
    \caption{Fundraising Matching Grant Experiment - External Validity}
    \begin{tabular}{cccccc}
    \toprule
          \multicolumn{3}{c}{$\theta_0=3.34$}  & \multicolumn{3}{c}{$\theta_1=3.56$} \\
          \cmidrule(lr){1-3}\cmidrule(lr){4-6}
 $\zeta_0$	&	$\nu_0$	&	$\alpha_0$	&	$\zeta_0$	&	$\nu_0$	&	$\alpha_1$	\\
0	    &	0.01	&	0.013	&	0	&	0.01	&	0.038	\\
3.42	&	782	    &	0.646	&	3.44	&	252	&	0.869	\\
3.42	&	0.01	&	0.014	&	3.44	&	0.01	&	0.041	\\
3.11	&	284	    &	0.313	&	3.27	&	223	&	0.012	\\
3.11	&	0.01	&	0.014	&	3.27	&	0.01	&	0.014	\\
             \bottomrule
    \end{tabular}%
  \label{Table:alpha}%

  \begin{tablenotes}
    \scriptsize{
      Notes: Notes:  This table reports the $\alpha$ corresponding to the initial priors when re-simulating the Bill Melinda Gates Foundation Experiment \citep{Karlan_List:2020}, with $\epsilon=0.30$. Each simulation lasted for at most 600 periods, and the results are averaged over 1,000 simulations. For the multi-prior models, we consider 5 sets of priors, corresponding to: $\zeta^0_0 = [0,0], \nu=[0.01,0.01]$, $\zeta^1_0 = [3.424909, 3.4407649], \nu=[782,252]$, $\zeta^2_0 = [3.424909, 3.4407649], \nu=[0.01,0.01]$, $\zeta^3_0 = [3.106395, 3.2722909], \nu=[284,223]$, $\zeta^4_0 = [3.106395, 3.2722909], \nu=[0.01,0.01]$. For the stopping rule, we set $B=100$.
    }
    \end{tablenotes}
    \end{threeparttable}
\end{table}%


==> tab_app.tex <==
% Table generated by Excel2LaTeX from sheet 'Main '
\begin{table}[ht]
  \centering
  \small
    \begin{threeparttable}
    \caption{Fundraising Matching Grant Experiment}
    \begin{tabular}{lcccccc}
    \toprule
          & \multicolumn{1}{c}{RCT}  & \multicolumn{4}{c}{$\alpha$-Model} \\
          \cmidrule(lr){2-2}\cmidrule(lr){3-6}
          & (1)   & (2)   & (3)   & (4)   & (5)  \\
          \hline
$\epsilon$-Greedy	&	1	&	0.2	&	0.25	&	0.3	&	0.35	\\
Average Stopping Period	&	600	&	198.29	&	171.492	&	180.579	&	182.348	\\
Probability of Making a Mistake at Stopping Period	&	0.006	&	0.024	&	0.027	&	0.028	&	0.029	\\
Average Payoffs	&	2071.57	&	2127.94	&	2127.87	&	2126.12	&	2125.46	\\
$10^{th}$ Quantile of Payoff Distribution	&	2032.11	&	2106.23	&	2108.70	&	2104.645	&	2102.71	\\
$50^{th}$ Quantile of Payoff Distribution	&	2072.69	&	2131.21	&	2131.15	&	2129.36	&	2129.60	\\
$90^{th}$ Quantile of Payoff Distribution	&	2109.09	&	2149.75	&	2149.75	&	2149.75	&	2149.75	\\
    \bottomrule
    \end{tabular}%
  \label{Table:app}%

  \begin{tablenotes}
    \scriptsize{
      Notes:  This table reports the results of re-simulating the Bill Melinda Gates Foundation Experiment \citep{Karlan_List:2020}. Each simulation lasted for at most 600 periods, and the results are averaged over 1,000 simulations. In column 1, we report the results for a standard randomized control trial. In columns 2-5, we report the results for several multi-prior models with different degrees of experimentation, as indicated by $\epsilon$. For the multi-prior models, we consider 5 sets of priors, corresponding to: $\zeta^0_0 = [0,0], \nu=[0.01,0.01]$, $\zeta^1_0 = [3.424909, 3.4407649], \nu=[782,252]$, $\zeta^2_0 = [3.424909, 3.4407649], \nu=[0.01,0.01]$, $\zeta^3_0 = [3.106395, 3.2722909], \nu=[284,223]$, $\zeta^4_0 = [3.106395, 3.2722909], \nu=[0.01,0.01]$. For the stopping rule, we set $B=100$.
    }
    \end{tablenotes}
    \end{threeparttable}
\end{table}%


==> tab_app_v2.tex <==
% Table generated by Excel2LaTeX from sheet 'Main '
\begin{table}[ht]
  \centering
  \small
    \begin{threeparttable}
    \caption{Fundraising Matching Grant Experiment}
    \begin{tabular}{lcccccccccc}
    \toprule
          & \multicolumn{1}{c}{RCT}  & \multicolumn{4}{c}{$\alpha$-Model} & \multicolumn{4}{c}{Non-$\alpha$ Model}\\
          \cmidrule(lr){2-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}
          & (1)   & (2)   & (3)   & (4)   & (5) & (6)   & (7)   & (8)   & (9) \\
          \hline
$\epsilon$-Greedy	&	1	&	0.2	&	0.25	&	0.3	&	0.35 &	0.2	&0.25& 0.3&0.35	\\
Average Stopping Period	&	600	&	198.3	&	171.5	&	180.6	&	182.4	&	548.8	& 527.5	&	511.6	&	509.2 \\
Probability of Making a Mistake at Stopping &	0.006	&	0.024	&	0.027	&	0.028	&	0.029	&	0.033	&	0.022	&	0.028	&	0.022\\
Average Payoffs	&	2071.57	&	2127.94	&	2127.87	&	2126.12	&	2125.46	&	2117.05	&	2116.97	&	2112.32	&	2111.30\\
$10^{th}$ Quantile of Payoff Distribution	&	2032.11	&	2106.23	&	2108.70	&	2104.645	&	2102.71	&	2079.99	&	2080.34	&	2073.30	&	2074.08\\
$50^{th}$ Quantile of Payoff Distribution	&	2072.69	&	2131.21	&	2131.15	&	2129.36	&	2129.60	&	2118.51	&	2118.63	&	2114.34	&	2113.83 \\
$90^{th}$ Quantile of Payoff Distribution	&	2109.09	&	2149.75	&	2149.75	&	2149.75	&	2149.75	&	2153.62	&	2153.62	&	2153.62	&	2153.62	\\
    \bottomrule
    \end{tabular}%
  \label{Table:app}%

  \begin{tablenotes}
    \scriptsize{
      Notes:  This table reports the results of re-simulating the Bill Melinda Gates Foundation Experiment \citep{Karlan_List:2020}. Each simulation lasted for at most 600 periods, and the results are averaged over 1,000 simulations. In column 1, we report the results for a standard randomized control trial. In columns 2-5, we report the results for several multi-prior models with different degrees of experimentation, as indicated by $\epsilon$. For the multi-prior models, we consider 5 sets of priors, corresponding to: $\zeta^0_0 = [0,0], \nu=[0.01,0.01]$, $\zeta^1_0 = [3.424909, 3.4407649], \nu=[782,252]$, $\zeta^2_0 = [3.424909, 3.4407649], \nu=[0.01,0.01]$, $\zeta^3_0 = [3.106395, 3.2722909], \nu=[284,223]$, $\zeta^4_0 = [3.106395, 3.2722909], \nu=[0.01,0.01]$. For the stopping rule, we set $B=100$, In columns 6-10, we report the results for models with different degrees of experimentation, as indicated by $\epsilon$, but no priors.
    }
    \end{tablenotes}
    \end{threeparttable}
\end{table}%

